Code-centric Learning-based Just-In-Time Vulnerability Detection

Attacks against computer systems exploiting software vulnerabilities can cause substantial damage to the cyber-infrastructure of our modern society and economy. To minimize the consequences, it is vital to detect and fix vulnerabilities as soon as possible. Just-in-time vulnerability detection (JIT-VD) discovers vulnerability-prone ("dangerous") commits to prevent them from being merged into source code and causing vulnerabilities. By JIT-VD, the commits' authors, who understand the commits properly, can review these dangerous commits and fix them if necessary while the relevant modifications are still fresh in their minds. In this paper, we propose CodeJIT, a novel code-centric learning-based approach for just-in-time vulnerability detection. The key idea of CodeJIT is that the meaning of the code changes of a commit is the direct and deciding factor for determining if the commit is dangerous for the code. Based on that idea, we design a novel graph-based representation to represent the semantics of code changes in terms of both code structures and program dependencies. A graph neural network model is developed to capture the meaning of the code changes represented by our graph-based representation and learn to discriminate between dangerous and safe commits. We conducted experiments to evaluate the JIT-VD performance of CodeJIT on a dataset of 20K+ dangerous and safe commits in 506 real-world projects from 1998 to 2022. Our results show that CodeJIT significantly improves the state-of-the-art JIT-VD methods by up to 66% in Recall, 136% in Precision, and 68% in F1. Moreover, CodeJIT correctly classifies nearly 9/10 of dangerous/safe (benign) commits and even detects 69 commits that fix a vulnerability yet produce other issues in source code

==> 2.background.tex <==
\section{Background}
\label{sec:background}

In this section, we will introduce relevant key concepts relating to code representations, graph neural networks (GNNs), and GNN model interpretation.

\textbf{Vulnerability-related Commits}. \textit{Vulnerability Contributing Commits (VCCs)} are the commits that introduce a vulnerability in the code after applying the code changes. In the existing studies~\cite{vccfinder,vuldigger}, VCCs are collected by finding the commits introduced vulnerabilities in the code that then are fixed by another reported commit (safe/clean commits, so-called \textit{Vulnerability Fixing Commits - VFCs}). In fact, a vulnerability in the code might require multiple commits to be formed over time. \textit{Vulnerability Triggering Commits (VTCs)} are the last VCC that exposes the unexpected behaviors. To avoid frustrating and providing developers false-alarm warnings, we focus on detecting VTCs to warn developers right before vulnerabilities are completely formed. 


\textbf{Source Code Representation}. In the literature, the code representations are classified into three main categories: token-based, tree-based, and graph-based. 
%
\textit{Token-based representation} treats source code as free text. This technique converts the code into a list of tokens where each word (e.g., \texttt{getSalary}) is a token, but each keyword (\texttt{void}) or special character (e.g., \texttt{(}) is also a token. 
%
\textit{Tree-based representation} carries the syntactical information of the code via the abstract syntactic structure of the code such as Abstract Syntax Tree (AST). AST is widely used by the tools for many SE tasks. With the \textit{graph-based} approaches, the semantic information of the source code is represented through graphs in various levels. Control Flow Graph (CFG) expresses the execution flow of the program. Meanwhile, the program (data/control) dependencies of the code are captured by a Program Dependency Graph (PDG).

\textbf{Graph Neural Network (GNN)}. Recently, GNNs have demonstrated superior performance in many software engineering tasks such as vulnerability detection~\cite{velvet,linevd,ivdetect}, clone detection~\cite{?}, and bug fixing~\cite{?} where source code is modeled as graphs. GNNs learn to represent the graph structure whose nodes are defined by their neighbors and their connections. 

% \textbf{GNN Model Explainability}. Explainable machine learning or artificial intelligence (XAI), is experiencing rapid developments to tackle the opacity issue of deep learning techniques. Similarly for graph neural networks (GNNs), an increasing number of approaches have been proposed to provide explanations for GNNs or to improve GNN explainability. In general, XAI techniques could be categorized into Instance-level methods (provide explanations for each individual prediction) or Model-level approaches (provide explanations for the whole model). In this work, we focus on the instance-level approaches. These methods could be gradient or features-based methods, perturbation-based methods, decomposition methods, or surrogate.

\textbf{GNN Explanation}. Recently, an increasing number of approaches have been proposed to provide explanations for GNNs or to improve GNN explainability~\cite{yuan2022explainability}. In general, GNN explanation techniques could be categorized into instance-level methods (providing explanations for each individual prediction) or model-level approaches (providing explanations for the whole model). To produce the explanations for each case of (JIT-VD) GNN models, we focus on the instance-level approaches which are categorized into gradient/features-based, perturbation-based, decomposition, or surrogate methods~\cite{yuan2022explainability}.


==> 5.framework/5.1.vul_detection.tex <==
\subsection{Code-centric Just-In-Time Vulnerability Detection}
Fig.~\ref{fig:model} shows our JIT-VD model. In this work, we treat each CTG as a relational heterogeneous graph and thus apply relational graph attention networks~\cite{rgat} for the JIT-VD task.
%
% The model extracts the features to represent the nodes and edges in the constructed CTGs of the known commits. 



First, the nodes are embedded into $d$-dimensional hidden features $n_i$ produced by embedding the content of the nodes.
%
Then, to form the node feature vectors, the node embedding vectors are annotated the change operators (\textit{added}, \textit{deleted}, and \textit{remained}) by concatenating corresponding one-hot vector of the operators to the embedded vectors, $h^{0}_i = n_i \bigoplus \alpha(n_i)$, where $\bigoplus$ is the concatenating operator and $\alpha$ returns the one-hot vector corresponding the annotation of node $i$.
%
%
The resulting vectors are fed to a relational graph attention (RGAT) model.
%
%
Similar to general relational graph convolution network (RGCN)~\cite{rgcn}, each layer of RGAT computes the representations for the nodes of the graph through message passing, where each node gathers features from its neighbors under every relation to represent local graph structure. Stacking $L$ layers allows the network to build node representations from the $L$-hop neighborhood of each node.
% This guarantees the transformation to build local reception fields and be invariant to both graph size and vertex re-indexing.
%
%
Thus, the feature vector $h^{l+1}_{i}$ at node $i$ at the next layer in RGAT is: 
%
\begin{equation} \label{eq:propagate_rule}
h^{l+1}_{i} =\sigma \left( 
\sum_{r \in \mathcal{R}}
    \sum_{j \in \mathcal{N}^r_i} \frac{1}{c_{i,r}} g_j^r
\right)
\end{equation}
%
%
%
%
% h^{l+1}_{i} =\sigma \left( \sum_{j \in \mathcal{N}_i} \frac{1}{c_{ij}} h^{l}_{i} W^l \right)
%
% h^{l+1}_{i} =\sigma \left( 
% W^l_0 h^{l}_{i} + 
% \sum_{r \in \mathcal{R}}
%     \sum_{j \in \mathcal{N}^r_i} \frac{1}{c_{i,r}}  W^l_r h^{l}_{j} 
% \right)
%
%
%
where $g_j = W^l_r h^{l}_{j}$ is the distinct intermediate representation of node $j$ under relation $r$, $W^l_r$ is a learnable weight matrix for feature transformation specific for relation $r$. In Equation (\ref{eq:propagate_rule}), $\mathcal{N}^r_i$ is the set of neighbor indices of node $i$ under relation $r \in \mathcal{R}$.
% including \textit{structure}, \textit{execution flow}, \textit{dependency}, and \textit{self-connection} which is a single special relation from node $i$ to itself.
%
Additionally, $1/c_{i}^r$ is a problem-specific normalization constant that can be chosen in advance (such as $c_{i}^r = |\mathcal{N}_i^r|$). 
%
% $c_{ij} =\sqrt{|\mathcal{N}_i| \times |\mathcal{N}_j|}$ is a normalization constant based on graph structure, 
Meanwhile, $\sigma$ is a non-linear activation function such as ReLU.
%
In this work, instead of using constant $1/c_{i}^r = |\mathcal{N}_i^r|^{-1}$, we replace the normalization constant by an learnable attention weight $a_{ij}^r$, where $\sum_{j,r} a_{ij}^r = 1$, to allow the model learn the importance of node $j$ and the relation between node $i$ and node $j$ under relation $r$~\cite{rgat}:
%
% Particularly, 
%
$$
a_{ij}^r = \text{softmax}_{j}(E_{ij}^r) =  \frac{\exp{(E_{ij}^r)}}{\sum_{k \in \mathcal{N}^r_i} \exp{(E_{ik}^r)}} 
$$
%
%
$$
E_{ij}^r = \text{LeakyReLu}(q_i^r + k_j^r)
$$
%
$$
q_i^r = g_i^r Q^r, \text{ and } k_j^r = g_j^r K^r
$$
%
%
where $Q^r$ and $K^r$ are the query kernel and key kernel projecting $g_i$ (and $g_j$) into query and key representations~\cite{rgat}. $Q^r$ and $K^r$ are combined to form the attention kernel for relation $r$, $A^r = Q^r \bigoplus K^r$.

After $L$ RGAT layers, a $d$-dimensional graph-level vector representation $H$ for the whole CTG $\mathcal{G} = \langle \mathcal{N}, \mathcal{E}, \alpha \rangle$ is built by averaging over all node features in the final RGAT layer, $H = \frac{1}{|\mathcal{N}|} \sum_{i \in [1, |\mathcal{N}|]} h^L_i$. Finally, the graph features are then passed to a Multilayer perceptron (MLP) to classify if $\mathcal{G}$ is dangerous or not.

\begin{figure*}
    \centering
    \includegraphics[width=2.0\columnwidth]{imgs/model.png}
    \caption{Just-In-Time Vulnerability Detection Model}
    \label{fig:model}
\end{figure*}



















































































%SON OLD
% First, nodes and edges are embedded into $d$-dimensional hidden features $h_i$ and $e_{ij}$ produced by embedding the content of the nodes and edges.
% %
% Then, the node embedding vectors and and edge embedding vectors are annotated the change operators (\textit{added}, \textit{deleted}, and \textit{remained}) by concatenating the encoded vectors of the change operators to the embedded vectors, $h^{0}_i=concat(h^{0}_i, cop[h^{0}_i])$ and $e^{0}_{ij}=concat(e^{0}_{ij}, cop[e^{0}_{ij}])$.
% %
% %
% The resulting vectors are fed to a graph neural network (GNN) model. In this work, we treat each CTG as a renational heterogeneous graph, and use relational graph convolution network (R-GCN)~\cite{r-gnn} to classify the CTGs of commits. 
% %
% %
% In GCNs, each layer computes the representations for the nodes of the graph through message passing, where each node gathers features from its neighbors under every relation to represent local graph structure~\cite{?}. Stacking $L$ layers allows the network to build node representations from the $L$-hop neighborhood of each node.
% % This guarantees the transformation to build local reception fields and be invariant to both graph size and vertex re-indexing.
% %
% %
% Thus, the feature vector $h^{l+1}_{i}$ at node $i$ at the next layer in the R-GNN is: 
% %
% $$
% % h^{l+1}_{i} =\sigma \left( \sum_{j \in \mathcal{N}_i} \frac{1}{c_{ij}} h^{l}_{i} W^l \right)
% %
% h^{l+1}_{i} =\sigma \left( 
% W^l_0 h^{l}_{i} + 
% \sum_{r \in \mathcal{R}}
%     \sum_{j \in \mathcal{N}^r_i} \frac{1}{c_{i,r}}  W^l_r h^{l}_{j} 
% \right)
% %
% $$
% %
% where $\mathcal{N}^r_i$ is the set of neighbor indices of node $i$ under relation $r \in \mathcal{R} = \{\text{structure}, \text{execution flow}, \text{dependency}\}$, $c_{i,r}$ is a problem-specific normalization constant that can be chosen in advance (such as $c_{i,r} = |\mathcal{N}_i^r|$). 
% %
% $W^l_r$ is a learnable weight matrix for feature transformation specific for relation $r$, while $W^l_0$ is a linear projection via a learnable weight matrix for a single self-connection of a special relation
% type to node $i$,
% % $c_{ij} =\sqrt{|\mathcal{N}_i| \times |\mathcal{N}_j|}$ is a normalization constant based on graph structure, 
% and $\sigma$ is an non-linear activation function such as ReLU.
% %
% In this work, instead of using $1/c_{i,r}$ which is a constant, we replace by an learnable attention weight $a_{ij,r}$, where $\sum_{j,r} a_{ij,r} = 1$, to allow the model learn the importance of node $j$ and the relation between node $i$ and node $j$ under relation $r$~\cite{gat}. 
% %
% % Particularly, 
% % %
% % $$
% % \alpha_{ij,r} = softmax_{j,r}(e_{ij,r}) =  \frac{\exp{(e_{ij,r})}}{\sum_{j \in \mathcal{N}^r_i} \exp{(e_{ik,r})}} 
% % % \frac{\exp{e_{ij,r}}{}
% % % \sum_{j \in \mathcal{N}^r_i} \exp{e_{ik,r}}
% % $$
% %
% After $L$ R-GNN layers, a $d$-dimensional graph-level vector representation $X_\mathcal{G}$ for the whole CTG $\mathcal{G} = \langle \mathcal{N}, \mathcal{E}, \alpha \rangle$ is built by averaging over all node features in the final R-GCN layer, $X_\mathcal{G} = \frac{1}{|\mathcal{N}|} \sum_{i \in [0, |\mathcal{N}|]} h^L_i$. Finally, the graph features are then passed to a Multilayer perceptron (MLP) to classify if $\mathcal{G}$ is dangerous or not.

% \begin{figure*}
%     \centering
%     \includegraphics[width=2.0\columnwidth]{imgs/model.png}
%     \caption{Just-In-Time Vulnerability Detection Model}
%     \label{fig:model}
% \end{figure*}

==> 5.framework/5.2.vul_inspection.tex <==
\subsection{Integrated Just-In-Time Vulnerability Localization}
After a suspicious commit is detected by our JIT-VD model, to utilizing the insights from the model's decision-making process for narrowing down the search space for the dangerous changes, a model interpreter is employed to provide the explanations of the model's decision. The explanations should point down which parts (nodes and edges) in the CTG are the deciding elements for the model's conclusion. These important edges/nodes are use to identify the (un)changed code statements in the commit which suspiciously cause vulnerabilities in the code.
%
%

For a trained JIT-VD model and its prediction for a CTG $\mathcal{G} = \langle \mathcal{N}, \mathcal{E}, \mathcal{R}, \alpha \rangle$, an interpreter assigns an importance score to either each edge $e^r_{ij} \in \mathcal{E}$ or each node $n_i \in \mathcal{N}$ by the edge importance function or the node importance function. Formally, $\textit{IM}_\mathcal{N}: \mathcal{N} \to [0,1]$ and  $\textit{IM}_\mathcal{E}: \mathcal{E} \to [0,1]$, the higher $\textit{IM}_\mathcal{E}(e^r_{ij})$ and $\textit{IM}_\mathcal{N}(n_i)$, the more important edge $e$ and node $n$ to the model's prediction for $\mathcal{G}$.
%
%
%
Intuitively, a statement in $\mathcal{G}$ contains more important elements, then the statement is more suspicious. Thus, given the node importance function $\textit{IM}_\mathcal{N}$, the suspiciousness of a statement node, $s \in \mathcal{N}$ corresponding to a code statement is determined by summing the importance scores of all the AST descendants of $s$:
%
%
\begin{equation} \label{eq:suspiciousness}
% \mathscr{S}(s) = \max_{n \in \textit{Desc}(s)} \textit{IM}_\mathcal{N}(n)
\mathscr{S}(s) = \sum_{n \in \textit{Desc}(s)} \textit{IM}_\mathcal{N}(n)
\end{equation}
%
%
where $\textit{Desc}(s) \subset \mathcal{N}$ returns the set of AST descendant nodes of $s$, which can be collected by traversing $\mathcal{G}$ from $s$ on structure edges. Meanwhile, if the edge importance function $\textit{IM}_\mathcal{E}$ is provided instead of the node importance function, we derive the importance of a node $n \in \mathcal{N}$ as: 
%
%
\begin{equation} \label{eq:importance_node}
\textit{IM}_\mathcal{N}(n_i) = \max_{r \in \mathcal{R}} 
\left( 
\sum_{j \in \mathcal{N}^r_i} \textit{IM}_\mathcal{E}(e^r_{ij})
+
\sum_{k \in \mathcal{N}^{-r}_i} \textit{IM}_\mathcal{E}(e^r_{ki})
\right)
\end{equation}
%
%
where $\mathcal{N}^r_i$ is the set of neighbor indices of $n_i$ under relation $r \in \mathcal{R}$, while $\forall k \in \mathcal{N}^{-r}_i$, there is an edge $\langle n_i, r, n_k \rangle \in \mathcal{E}$. The intuition of (\ref{eq:importance_node}) is that $n_i$ is more important regarding a relation $r \in \mathcal{R}$ if there are more important $r$-edges directly relevant to $n_i$. The overall importance of $n_i$ is the highest importance score among the scores regarding all relations.


% This could be done by the perturbation-based GNN explanation techniques which is widely employed to explain GNN models. These techniques assume that important input parts significantly contribute to the decisions while unimportant parts have minor influences. Based on the model and its decision, these methods score the importance of the input parts.
%
%

% To derive explanations, the general goal of perturbation-based methods is to reduce redundant information in a graph which does not directly impact the model's decisions. For a CTG $\mathcal{G}$, the approaches find the compact sub-graph $\mathcal{G_S}$ of $\mathcal{G}$ that minimizes the deference in the prediction scores using $\mathcal{G}$ and $\mathcal{G_S}$. 
%
% This task is treated as generating a mask for edges/nodes/node features to explain the predictions via mask optimization. The masks are obtained in different methods with various objective functions to indicate the input importance. The generated masks are combined with $\mathcal{G}$ to obtain $\mathcal{G_S}$ containing important input information.
%
% Finally, $\mathcal{G_S}$ is fed into the trained JIT-VD model to evaluate the masks and update the mask generation methods.
%
% Intuitively, the masks should capture the important parts which convey the key semantic meaning of $\mathcal{G}$, and hence the model produces a similar prediction to the prediction for $\mathcal{G}$. 
%
%

In general, any GNN explanation technique e.g., GNNExplainer~\cite{gnn_explainer} or AttentionExplainer could be applied to provide $\textit{IM}_\mathcal{N}$ or $\textit{IM}_\mathcal{E}$.
%
% In this work, we apply GNNExplainer~\cite{gnn_explainer} which is a popular perturbation-based technique for the model explanation step in our framework. The masks are optimized by maximizing the mutual information between the predictions of $\mathcal{G}$ and the predictions of the newly obtained graph~\cite{gnn_explainer}.
%
The impact of selecting the explanation technique in our framework on vulnerability localization performance will be empirically shown in Section~\ref{sec:intrinsic}. 




% The resulting sub-graph $\mathcal{G_S}$ is directly used as an interpretation. We can similarly produce the interpretations for the cases of non-vulnerability result....(statement level)


% Generally, to derive explanations, the goal of perturbation-based approaches is to reduce redundant information in a graph which does not directly impact the model's decisions. For a CTG $\mathcal{G}$, the approaches find the minimal sub-graph $\mathcal{G_S}$ of $\mathcal{G}$ that minimizes the deference in the prediction scores using $\mathcal{G}$ and $\mathcal{G_S}$. Particularly, this task is treated as generating a mask for edges/nodes to explain the predictions via mask optimization. 
%
% The masks are optimized by maximizing the mutual information between the predictions of $\mathcal{G}$ and the predictions of the newly obtained graph.

==> 7.results/intrinsic/feature_engineering.tex <==
\subsubsection{Impact of Feature Engineering}
\begin{table}[]
\centering
\caption{Impact of Feature Engineering}
\label{tab:feature_engineering}
\begin{tabular}{@{}lrrrrr@{}}
\toprule
                        & \textit{Precision} & \textit{Recall}   & \textit{F1}   & \textit{Accuracy} \\ \midrule
Word2vec                 & XXX               & XXX          & XXX                 & XXX               \\
FastText                & XXX               & XXX          & XXX                & XXX                \\
CodeBERT         & XXX	             & XXX         & XXX	             & XXX	             \\
\bottomrule
\end{tabular}
\end{table}

==> 7.results/intrinsic/predic_model.tex <==
\begin{table}[]
\centering
\caption{Impact of Prediction Model}
\label{tab:predict_model}
\begin{tabular}{@{}lrrrrr@{}}
\toprule
                        & \textit{Precision} & \textit{Recall}   & \textit{F1}   & \textit{Accuracy} \\ \midrule
MLP                & XXX               & XXX          & XXX                 & XXX               \\
Logistic Regression                 & XXX               & XXX          & XXX                & XXX                \\
Gradient Boosting Machine          & 0.82	             & 0.66	         & 0.73	             & 0.85	             \\
Random Forest   & 0.86	             & 0.62	         & 0.72	             & 0.85	             \\
\bottomrule
\end{tabular}
\end{table}

==> [TSE'23] Just-In-Time Software Vulnerability Detection/0.abstract.tex <==
\begin{abstract}
% Software is a critical element in a broad range of real-world systems. 
Attacks against computer systems exploiting software vulnerabilities can cause substantial damage to the cyber-infrastructure of our modern society and economy.
To minimize the consequences, it is vital to detect and fix vulnerabilities as soon as possible. 
%
Just-in-time vulnerability detection (JIT-VD) discovers vulnerability-prone (``dangerous") commits to prevent them from being merged into source code and causing vulnerabilities. By JIT-VD, the commits' authors, who understand the commits properly, can review these dangerous commits and fix them if necessary while the relevant modifications are still fresh in their minds.
%
%
%
%
In this paper, we propose \tool, a novel code-centric learning-based approach for just-in-time vulnerability detection. 
%
The key idea of \tool is that \textit{the meaning of the code changes of a commit is the direct and deciding factor for determining if the commit is dangerous for the code.}
%
%
Based on that idea, we design a novel graph-based representation to represent the semantics of code changes in terms of both code structures and program dependencies. 
%
% Based on that idea, we design a novel graph-based representation to represent the code changes in terms of  both syntactic, i.e., code structures, and semantic, i.e., program dependencies. 
%
A graph neural network model is developed to capture the meaning of the code changes represented by our graph-based representation and learn to discriminate between dangerous and safe commits. 
%
We conducted experiments to evaluate the JIT-VD performance of \tool on a dataset of 20K+ dangerous and safe commits in 506 real-world projects from 1998 to 2022. Our results show that \tool significantly improves the state-of-the-art JIT-VD methods by up to 66\% in Recall, 136\% in Precision, and 68\% in F1. 
%
Moreover, \tool correctly classifies nearly 9/10 of dangerous/safe (benign) commits and even detects 69 commits that fix a vulnerability yet produce other issues in source code.


\end{abstract}


==> [TSE'23] Just-In-Time Software Vulnerability Detection/1.intro.tex <==
\section{Introduction}

Software is a critical element in a broad range of real-world systems. Attacks against computer systems exploiting software vulnerabilities (security defects/bugs), especially in critical systems such as traffic control, aviation coordination, chemical/nuclear industrial operation, and national security systems, can cause substantial damage. 
%
The latest survey~\cite{survey_3} in 2021 shows that by 2020, the total cost of bugs related to software vulnerabilities in the US (accounting for 33\% of the market share in the whole world technology market) is 1.56 trillion USD. 
This cost accounts for 75\% of the cost caused by poor-quality software.
%
To minimize the consequences caused by vulnerabilities in software, vulnerabilities should be detected and fixed as soon as possible because late detection and correction can cost up to 200 times as much as early correction or even cause more severe damage~\cite{jit_vul_less_is_more,jit_bug,jit_vul_survey}. 
%
The most popular and effective solution being applied in practice is to use techniques that scan the entire source code and automatically detect the presence of vulnerabilities before the software is released~\cite{survey_papers,ese_empirical}. 

Most of the existing methods scan all the software components such as files, functions, or lines in source code to detect vulnerabilities~\cite{survey_papers,linevd,linevul,ivdetect,velvet,vuldeeppeaker,mu_vuldeeppeker,devign,vulsniper,mvd,issta_22}. These scanning techniques often report a large number of alarms and multiple of them are false alarms~\cite{kang2022detecting, ngo2021ranking}. After that, the detected suspicious components still need to be manually examined to determine the actual presence of the vulnerability. 
%
Such task requires selecting an \textit{appropriate developer group} who can thoroughly understand the business logic of the components.
% last changes applied to the source code. 
%
%
%
However, this proper developer selection task is also very challenging~\cite{jit_vul_less_is_more,jit_bug,jit_vul_survey}.
%
In practice, developers usually commit their changes very regularly. In Mozilla Firefox, the developers recently pushed 10K+commits to construct a release from the previous version~\footnote{From \texttt{release\_v109} to \texttt{release\_v110}, more details: \url{https://github.com/mozilla-mobile/fenix}}. 
%
At the same time, we found that there are some files touched by up to 155 developers in Mozilla Firefox. Thus, with large accumulated sets of commits and authors at the released time, correctly identifying the authors of dangerous code could be non-trivial~\cite{vccfinder, jit_bug,jit_vul_less_is_more,szz}. 
Even if the authors are correctly identified, the developers might still need to spend much time recalling and drilling down to the files/functions. This could significantly slow down the quality assurance process and development cycle.
Thus, although the recommendations based on vulnerability detection at the release time (long-term recommendations) can be useful in some contexts, they have their own drawbacks in practice~\cite{jit_bug,jit_vul_less_is_more,jit_vul_survey}. 
%

Meanwhile, \textit{\jit}~or \textit{commit-level} recommendations (short-term recommendations) could be preferred because they allow commits' authors to get immediate feedback on their code changes. This feedback could help developers faster improve their code quality since the context of the changes is still fresh in their minds. In addition, the \jit vulnerability detection techniques facilitate not only the authors in responsibly making code changes but also code auditors in reviewing code commits~\cite{jit_vul_less_is_more,ese_empirical}. 
%

The past few years have witnessed a few successful research to investigate \textit{\jit vulnerability detection}~\cite{vuldigger,vccfinder} and \jit general defect detection~\cite{jitline, jit-fine,lapredict,deepjit}.
% However, existing studies have several limitations. 
%
%
These studies utilize commit messages and expert features such as authors' experiences, commit time, and code changes' complexity (e.g., numbers of added/deleted lines of code) to calculate the metrics to determine if commits are suspicious. 
%
In fact, these features might have some correlations but not necessarily cause the presence of vulnerabilities at the commit level. For example, a commit whose message contains bug-fixing keywords such as ``\textit{fix}", ``\textit{failures}", or ``\textit{resolves}" could be very likely to be classified as a safe one~\cite{lapredict}. 
%
Although the commit fixes some bugs, the possibility that the commit creates other bugs in the code should not be eliminated.
%
Meanwhile, the studies utilizing the expert features often leverage on certain hypotheses~\cite{vccfinder,jitline,jit-fine,are_we_there,lapredict} such as the larger number of added lines of code, the higher possibility the commits contain vulnerabilities~\cite{lapredict}. Consequently, the dangerous commits with a few added lines of code could be misidentified.
% This possibility might be not determined by considering commit messages or the expert features.
%
% Thus, commit messages and the experts features could be important but they might not correctly reveal the vulnerabilities of code changes, which indeed exist inside the source code.
%
Thus, commit messages and the expert features could correlate but not necessarily result in the presence of vulnerabilities, which are, in fact, brought about by code changes.
% which are inside the source code.







In this paper, we introduce \tool, a novel \textit{\textbf{code-centric}} learning-based approach which focuses on capturing the meaning of code changes in known dangerous or safe (benign) commits, rather than utilizing commit messages or the expert features, to detect vulnerabilities at the commit level.
%
Our idea is that \textit{for a commit, the meaning of the changes in the source code is the direct and deciding factor for assessing the commit's suspiciousness.}
%
%
% This idea is reasonable because a commit is considered suspicious (i.e., can cause vulnerabilities) if its code changes could carry vulnerabilities, or introduce vulnerabilities when these changes are merged into the source code and interact with their related unchanged code. 
%
This idea is reasonable because a commit should be considered dangerous if its code changes carry vulnerabilities or interact with the unchanged code to collectively introduce vulnerabilities once the changed code is merged into the source code. 
%
% This idea is reasonable because a commit should be considered dangerous if its code changes carry vulnerabilities, or introduce the vulnerabilities exposed when the changed code is merged into the source code and interact with the unchanged code. 
% introduce the related code which can interact with the unchanged parts of the project and expose the vulnerabilities.
%
%

To implement our code-centric idea for JIT-VD, we propose a novel graph-based code transformation representation (\textbf{C}ode \textbf{T}ransformation \textbf{G}raph - CTG) to capture the semantics of the code changes caused by commits by representing the changed code in relation to the related unchanged code. Particularly, the CTG of a commit expresses the code changes/transformations in both the code structure and dependencies which are necessary to capture the syntax and semantics of the code changes.
%
Based on the code before and after the commit, the CTG is constructed from the set of nodes which are \textit{added}, \textit{deleted}, and \textit{unchanged} code elements such as statements, expressions, or operators. The CTG's nodes are connected by the edges which are the \textit{added}, \textit{deleted}, and \textit{unchanged} structure and dependency relations between the nodes.
%
%
Next,
% instead of additionally utilizing commit messages and the expert features like in the existing methods~\cite{vccfinder, vuldigger, jit-fine,jitline,deepjit},
\tool relies on the code-related aspects of commits, which are represented by their CTGs, to learn discriminating dangerous/safe commits. Particularly, CTGs can be intuitively treated as relational graphs. A Relational Graph Convolutional Network (RGCN) model is developed to capture the knowledge from the CTGs of the prior known safe/dangerous commits and learn to detect dangerous commits. 
%


We conducted experiments to evaluate the JIT-VD performance of {\tool} on a large dataset of 20K+ dangerous/safe commits in 506 C/C++ projects from 1998 to 2022. We compared {\tool} with the state-of-the-art JIT-VD approaches~\cite{vccfinder, deepjit, jitline, lapredict, jit-fine}. 
%
Our results show that \tool significantly improves the state-of-the-art JIT-VD techniques by up to 68\% in F1 and 77\% in classification accuracy. Especially, \tool can correctly distinguish nearly 9/10 of dangerous/safe commits. The recall of \tool is up to 66\% better than that of the existing approaches. Moreover, \tool can achieve the precision of 90\%, which is 32--123\% better than the precision of the other approaches. In other words, 9/10 suspicious commits detected by \tool actually are dangerous. Hence, with \tool, practitioners could discover more the commits dangerous for their code and spend less undesirable efforts for the false alarms during the security inspection process.
%

%
In brief, this paper makes the following contributions:

\begin{enumerate}
    \item Code Transformation Graph: A novel graph-based representation of code changes to capture the changes in the crucial aspects of code: the code structure and program dependencies. 
    \item {\tool}: A novel code-centric approach for detecting vulnerabilities at the commit level.
    \item An extensive experimental evaluation showing the performance of {\tool} over the state-of-the-art methods for just-in-time vulnerability detection.
    \item A public dataset of 20K+ safe and dangerous commits collected from 506 real-world projects, which can be used as a benchmark for evaluating related work.
\end{enumerate}
%
The detailed implementation of \tool and dataset can be found at: \textit{\url{https://github.com/ttrangnguyen/CodeJIT}}.



==> [TSE'23] Just-In-Time Software Vulnerability Detection/2.background.tex <==
\section{Background}
\label{sec:background}

In this section, we will introduce relevant key concepts relating to code representations, graph neural networks (GNNs), and GNN model interpretation.

\textbf{Vulnerability-related Commits}. \textit{Vulnerability Contributing Commits (VCCs)} are the commits that introduce a vulnerability in the code after applying the code changes. In the existing studies~\cite{vccfinder,vuldigger}, VCCs are collected by finding the commits introduced vulnerabilities in the code that then are fixed by another reported commit (safe/clean commits, so-called \textit{Vulnerability Fixing Commits - VFCs}). In fact, a vulnerability in the code might require multiple commits to be formed over time. \textit{Vulnerability Triggering Commits (VTCs)} are the last VCC that exposes the unexpected behaviors. To avoid frustrating and providing developers false-alarm warnings, we focus on detecting VTCs to warn developers right before vulnerabilities are completely formed. 


\textbf{Source Code Representation}. In the literature, the code representations are classified into three main categories: token-based, tree-based, and graph-based. 
%
\textit{Token-based representation} treats source code as free text. This technique converts the code into a list of tokens where each word (e.g., \texttt{getSalary}) is a token, but each keyword (\texttt{void}) or special character (e.g., \texttt{(}) is also a token. 
%
\textit{Tree-based representation} carries the syntactical information of the code via the abstract syntactic structure of the code such as Abstract Syntax Tree (AST). AST is widely used by the tools for many SE tasks. With the \textit{graph-based} approaches, the semantic information of the source code is represented through graphs in various levels. Control Flow Graph (CFG) expresses the execution flow of the program. Meanwhile, the program (data/control) dependencies of the code are captured by a Program Dependency Graph (PDG).

\textbf{Graph Neural Network (GNN)}. Recently, GNNs have demonstrated superior performance in many software engineering tasks such as vulnerability detection~\cite{velvet,linevd,ivdetect}, clone detection~\cite{?}, and bug fixing~\cite{?} where source code is modeled as graphs. GNNs learn to represent the graph structure whose nodes are defined by their neighbors and their connections. 

% \textbf{GNN Model Explainability}. Explainable machine learning or artificial intelligence (XAI), is experiencing rapid developments to tackle the opacity issue of deep learning techniques. Similarly for graph neural networks (GNNs), an increasing number of approaches have been proposed to provide explanations for GNNs or to improve GNN explainability. In general, XAI techniques could be categorized into Instance-level methods (provide explanations for each individual prediction) or Model-level approaches (provide explanations for the whole model). In this work, we focus on the instance-level approaches. These methods could be gradient or features-based methods, perturbation-based methods, decomposition methods, or surrogate.

\textbf{GNN Explanation}. Recently, an increasing number of approaches have been proposed to provide explanations for GNNs or to improve GNN explainability~\cite{yuan2022explainability}. In general, GNN explanation techniques could be categorized into instance-level methods (providing explanations for each individual prediction) or model-level approaches (providing explanations for the whole model). To produce the explanations for each case of (JIT-VD) GNN models, we focus on the instance-level approaches which are categorized into gradient/features-based, perturbation-based, decomposition, or surrogate methods~\cite{yuan2022explainability}.


==> [TSE'23] Just-In-Time Software Vulnerability Detection/3.example.tex <==
\section{Motivating Example}
\label{sec:example}
We first illustrate the problem of \jit vulnerability detection and explain the motivation for our solution.

\subsection{Observations}

\begin{figure}
% https://github.com/ffmpeg/ffmpeg/commit/2c635fabbf7ec8ed4f30d9b3c04d5c24cb7a081d
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=1\columnwidth]{imgs/c_1.png}
        \caption{Commit \texttt{2c635fa} fixing a vulnerability yet causing another}
        \label{fig:fixing-vt}
     \end{subfigure}
     \hfill

% % https://github.com/ffmpeg/ffmpeg/commit/ac480cb58dbe7859c96a08e9e5cd3dd3b0fb0ae7     
     \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=1\columnwidth]{imgs/c1_1.png}
        \caption{Commit \texttt{ac480cb} fixing the vulnerability in Fig.~\ref{fig:fixing-vt}}
        \label{fig:fixing}
     \end{subfigure}
     
    % \caption{Two commits in \textit{FFmpeg} project}
    \caption{Two commits in \textit{FFmpeg} project demonstrating the importance of understanding code changes for JIT-VD.}
\end{figure}




\textbf{Observation 1}. \textit{For a commit, the code changes' meaning is the reliable factor for deciding if the commit is dangerous or not}. 
Intuitively, a commit is dangerous to source code if it contains dangerous code changes either having vulnerabilities 
%
%
or introducing the vulnerabilities caused by the interaction between the changed code and the unchanged code.
%
%
%
For example, the commit in Fig.~\ref{fig:fixing-vt} contains vulnerable changed code itself, while the commit in Fig.~\ref{fig:vt2} brings a vulnerability to source code due to the relation between the changed and the unchanged code.
% For example, 
Specifically, in Fig.~\ref{fig:fixing-vt}, the added code itself contains a memory leak issue. 
%
The commit replaces the function call \texttt{avio\_read()} (at line 462, the old version) by a \texttt{if}-block examining the returned value of the call (lines 463--464, the new version). In the new version, \texttt{avio\_read()} allocates the memory of \texttt{st->codec->extradata}, yet the author forgot to free \texttt{extradata} when the values of \texttt{ret} and \texttt{len} are different (line 463 in the new version). 
%
In Fig.~\ref{fig:vt2}, 
adding \texttt{av\_free\_packet(\&pkt)} (line 1352, the new version) to free the packet data allocated by calling \texttt{av\_read\_frame} at line 1346 only when decoding audio frames. Consequently, the added code and the existing code collectively cause a leak problem.


Besides the code changes, to determine if a commit is suspiciously dangerous, ones could rely on expert features and commit messages~\cite{lapredict,vccfinder,jit-fine,jitline}.
%
Commit messages and expert features such as commit authors' experience or the number of added lines might have some relations to the suspiciousness of commits. However, they might be not necessarily discriminative for detecting dangerous commits. For example, safe commits and dangerous commits could have the same number of added lines, and be produced by the same author (e.g., the dangerous commit in Fig.~\ref{fig:fixing-vt} and the safe one in Fig.~\ref{fig:fixing}).
The application of commit messages and the expert features for JIT-VD is discussed in Sec.~\ref{sec:results}.
%







% For example, the dangerous commit in Fig.~\ref{fig:fixing-vt} and the safe (fixing) commit in Fig.~\ref{fig:fixing} are pushed by the same author and have the similar numbers of added lines.
% %
% %
% Meanwhile, \textit{commit messages could be also not reliable for JIT-VD}.
% %
% Zeng~\etal~\cite{lapredict} show that the message of a commit could provide the intent of the commit.
% %
% For example, if a commit's message contains ``\textit{failures}'', ``\textit{fix}'', ``\textit{resolves}'', or ``\textit{task-number}'', then the commit is more likely to be a fixing commit. 
% %
% However, developers often unintentionally bundle unrelated changes with different purposes (e.g., bug fix and refactoring) in a single commit (tangled commit)~\cite{untangling}.  
% %
% Multiple studies have shown that fixing a bugs is likely to result in another bug~\cite{guo2010characterizing, purushothaman2005toward}. We also found that various vulnerability-fixing commits actually cause other vulnerabilities.
% %
% For example, the commit shown in Fig.~\ref{fig:fixing-vt} is dangerous, yet has a message showing its \textit{bug-fixing} intention: \textit{``\textbf{Fixes} use of uninitialized memory''}.
% %
% %
% %
% The commit adds the check for \texttt{avio\_read()} result by removing line 462 in the old version and adding lines 463--464 in the new version to fix the use of uninitialized memory when the call is failed. 
% % %
% However, as show earlier, this unintentionally causes a memory leak. This issue is fixed by commit \texttt{ac480cb} shown in Fig.~\ref{fig:fixing} adding the call of \texttt{av\_free} to free \texttt{extradata} and setting \texttt{extradata\_size = 0} (lines 464--465 of the new version).
% %
% %
% %
% %
% Moreover, in practice, commit messages are often poor-quality, even empty~\cite{good_commit_message}. This makes the application of commit messages for detecting vulnerabilities at the commit level much less reliable.

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=0.9\columnwidth]{imgs/c.png}
        \caption{Commit \texttt{7328c2f} causing a vulnerability in \textit{FFmpeg}}
        \label{fig:vt2}
     \end{subfigure}
     \hfill

     \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=0.9\columnwidth]{imgs/c1.png}
        \caption{Commit \texttt{4fd1e2e} fixing the issue in Fig.~\ref{fig:vt2}}
        \label{fig:fixing2}
     \end{subfigure}
     
    % \caption{Example of a dangerous commit and its corresponding fixing commit}
    \caption{Two commits in \textit{FFmpeg} project demonstrating the importance of considering both changed and unchanged code in understanding code changes}
\end{figure}


\textbf{Observation 2}. \textit{To precisely capture the semantics of code changes, besides the changed parts, the unchanged code is also necessary}. 
%
%
Indeed, the unchanged code could connect the related changed parts and help to understand the code changes as whole. 
%
In Fig.~\ref{fig:ex_unchange}, without considering the unchanged parts (e.g., line 47, the old version/line 48, the new version), the changed parts (lines 25 and 49, the new version) can be considered as semantically irrelevant. However, the added lines 24--25 affect the behavior of the added line 49 via the unchanged statement (line 48, the new one). 


\begin{figure}[!h]
    \centering
    \includegraphics[width=0.75\columnwidth]{imgs/ex_unchanged.png}
    \caption{Unchanged code connects changed parts}
    \label{fig:ex_unchange}
\end{figure}


Additionally, once changed statements are introduced to a program, they change the program's behaviors by interacting with the unchanged statements via certain code relations such as control/data dependencies. 
%
% Hence, unchanged parts are necessary to precisely understand the meaning of different changes.
%
Hence, precisely distinguishing similar changed parts could require their relations with the unchanged parts. 
%
For example, although the atomic changes adding \texttt{av\_free\_packet(\&pkt)} in Fig.~\ref{fig:vt2} and Fig.~\ref{fig:fixing2} are apparently similar, they are semantically different in their related unchanged parts. 
%
Adding \texttt{av\_free\_packet(\&pkt)} in Fig.~\ref{fig:vt2} is to free the packet data only when decoding audio frames, which causes a leak problem after \texttt{7328c2f}. Meanwhile, the adding one in Fig.~\ref{fig:fixing2} (line 1353, the new version) at each demuxing loop iteration, not only when decoding. This safe commit fixes the unintentional problem caused by the dangerous commit \texttt{7328c2f} in Fig.~\ref{fig:vt2}.
%
%
%
The suspiciousness of commit \texttt{7328c2f} (Fig.~\ref{fig:vt2}) and commit \texttt{4fd1e2e} (Fig.~\ref{fig:fixing2}) could not be determined without considering the relation between the changed code and the unchanged code. 
% To determine the suspiciousness of commits, considering only the changed statements is insufficient.
%

Thus, \textit{not only the changed parts but also the related unchanged parts are necessary for representing code changes to precisely capture their meaning and determine their suspiciousness}.


\textbf{Observation 3}. \textit{The changes in both the code structure and dependencies are necessary and provide rich information for understanding and determining the suspiciousness of code changes}. 
%
For example, in Fig.~\ref{fig:fixing2}, the memory leaking issue is fixed by the changes in the dependencies of the function called \texttt{av\_free\_packet}. Indeed, changing the call of \texttt{av\_free\_packet} from line 1352 to line 1353 (outside the \texttt{if} block) causes the call no longer control-dependent on the \texttt{if}-statement (line 1349), and creates a new control dependency of the call on the \texttt{while}-statement at line 1346. 
%
As a result, instead of only when decoding (inside the \texttt{if} block), \texttt{av\_free\_packet} is always called in the \texttt{while}-loop to free the packet data. Thus, it is important to capture the dependency relation of the code changes.


%
Additionally, the \textit{Buffer Overflow} issue shown in Fig.~\ref{fig:example_change} is brought by the changes in the code structure. Specifically, while the dependencies between the statements remain unchanged, the right-hand-side of the comparison at line 4 is changed from \texttt{BUF\_SIZE} to \texttt{2*BUF\_SIZE}. This allows line 5 to copy the amount of data larger than the capacity of \texttt{buf}. This demonstrates the importance of the structure relation in understanding the code changes.



\textit{Overall}, these observations indicate that the code changes of a commit are the \textit{deciding factor} in determining the suspiciousness of the commit. To \textit{precisely} capture the changes' meaning, not only the changed code but also the related unchanged parts are required. The changes in the code structure and dependencies are essential to \textit{comprehensively} represent the meaning of the changes. 








\subsection{Key Ideas}
Based on the above observations, we introduce \tool 
centralizing the role of code changes in JIT-VD and considering the changed code of commits in relation to the unchanged code to assess commits' suspiciousness. For \tool to work, we rely on the following key ideas:


\begin{enumerate}
    
    \item We develop a graph-based representation for the code changes of commits, namely \textit{Code Transformation Graph (CTG)}. The representation captures the changes/transformations in both the code structure and dependencies of the changed code and the related unchanged code.

    \item A relational graph neural network model is employed to capture the knowledge of the known dangerous/safe commits represented in CTGs and evaluate the suspiciousness of newly-encountering commits.
    
\end{enumerate}






% \textbf{Vulnerability-related Commits}. \textit{Vulnerability Contributing Commits (VCCs)} are the commits which introduce a vulnerability in the code after applying the code changes. In the existing studies~\cite{vccfinder,vuldigger}, VCCs are collected by finding the commits introduced vulnerabilities in the code that then are fixed by another reported commit (safe/clean commits, so-called \textit{Vulnerability Fixing Commits - VFCs}). In facts, a vulnerability in the code might require multiple commits to be formed over time. \textit{Vulnerability Triggering Commits (VTCs)} are the last VCC which exposes the unexpected behaviors. To avoid frustrating and providing developers false-alarm warnings, we focus on detecting VTCs to warn developers right before vulnerabilities are completely formed. 




















































































































































% Meanwhile, commit messages could be also not reliable for the JIT-VD task. 
% %
% Zeng \etal~\cite{lapredict} show that the message of a commit could provide the intent of the commit and significantly impact JIT-VD models' predictions. For example, the commit is more likely to be a fixing commit if its message contains ``\textit{failures}'', ``\textit{fix}'', ``\textit{resolves}'', or ``\textit{task-number}''. 
% %
% In fact, developers often unintentionally bundle unrelated changes with different purposes (e.g., bug fix and refactoring) in a single commit (tangled commit)~\cite{untangling}.  
% %
% For example, the dangerous commit shown in Fig.~\ref{fig:fixing-vt} have a message showing its \textit{bug-fixing} intention: \textit{``\textbf{Fixes} use of uninitialized memory''}.
% %
% We found that several vulnerability-fixing commits actually cause other vulnerabilities. 
% %
% The commit in Fig.~\ref{fig:fixing-vt} adds the check for \texttt{avio\_read()} result by removing line 462 in the old version (left-hand line numbers) and adding lines 463--464 in the new version (right-hand line numbers) to fix the use of uninitialized memory when the call is failed. 
% %
% However, the author forgot to free \texttt{extradata} when \texttt{avio\_read()} is failed to be called. This unintentionally causes a memory leak. This issue is fixed by commit \texttt{ac480cb} adding the call of \texttt{av\_free} to free \texttt{extradata} and setting \texttt{extradata\_size = 0} (lines 464--465 of the new version).
% %
% Moreover, commit messages are often of poor quality, even empty~\cite{good_commit_message}. This makes the application commit message to detect vulnerabilities less reliable.

% Essentially, if a commit is dangerous, it contains dangerous code changes having vulnerabilities or causing vulnerabilities in the related code.
%
% However, understanding the semantic of code changes is difficult.









%SON: OLD

% \textbf{Observation 1}. \textit{Code is a reliable factor for deciding if a change is dangerous or not.} In general, to determine if a commit is suspiciously dangerous, ones could rely on expert features, commit messages, and commit code~\cite{lapredict,vccfinder,jit-fine}. 
% %
% We found that expert features such as commit authors or commit time might have some relations to dangerousness of commits, yet they are not sufficiently discriminative for detecting dangerous commits. For example, the dangerous commit in Fig.~\ref{fig:fixing-vt} and the clean/fixing commit in Fig.~\ref{fig:fixing} are pushed by the same author in a the same date (Jan 12, 2012).
% %
% Meanwhile, commit messages could be not reliable for the JIT-VD task. Indeed, Zeng \etal~\cite{lapredict} show that the message of a commit could provide the intent of the commit and significantly impact the model’s prediction results. For example, the commit is more likely to be a fixing commit if its message contains ``\textit{failures}'', ``\textit{fix}'', ``\textit{resolves}'', or ``\textit{task-number}''. However, developers often unintentionally bundle unrelated changes with different purposes (e.g., bug fix and refactoring) in a single commit (tangled commit)~\cite{untangling}. This makes the application commit message to detect vulnerabilities less reliable. 
% %
% %
% We found that several vulnerability-fixing commits actually cause other vulnerabilities. For example, the commit in Fig.~\ref{fig:fixing-vt} replaces \texttt{av\_destruct\_packet()} (line 1352) with \texttt{av\_free\_packet()} (line 1352) to resolve the ''over-free'' problems causing crashes when decoding audio frames. 
% %
% However, calling \texttt{av\_free\_packet()} at line 1352 causes a newly problem of leak in the containing function \texttt{show\_packets()}. Eventually, this issue is fixed by the commit shown in Fig.~\ref{fig:fixing} by moving the call to line 1353.
% %
% %
% % Moreover, utilizing commit messages and expert features might not provide the insight for security inspection...
% %
% %

% In fact, if a commit is vulnerable, it contains dangerous code changes having vulnerabilities or causing vulnerabilities in the related code.
% %
% However, understanding code changes is difficult.







% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\columnwidth]{imgs/c.png}
%     \caption{Commit \texttt{7328c2f} fixing a vulnerability yet causing another in \textit{FFmpeg}}
%     \label{fig:fixing-vt}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\columnwidth]{imgs/c'.png}
%     \caption{Commit \texttt{4fd1e2e} fixing the vulnerability in Fig.~\ref{fig:fixing-vt}}
%     \label{fig:fixing}
% \end{figure}


% \textbf{Observation 2}. \textit{Besides the changed parts, the unchanged code could carry important semantic change elements via syntactical, executional, and dependency relations}. 

% \textbf{Observation 2}. \textit{Besides the changed parts, the unchanged code could carry important semantic change elements via their relations}. 
% %
% For example, although the atomic changes adding \texttt{av\_free\_packet(\&pkt)} in Fig.~\ref{fig:fixing-vt} and Fig.~\ref{fig:fixing} are apparently similar, they are semantically different. 
% %
% Indeed, adding \texttt{av\_free\_packet(\&pkt)} in Fig.~\ref{fig:fixing-vt} is to correctly free the packet data when decoding audio frames. Not only when decoding, the adding one in Fig.~\ref{fig:fixing} at each demuxing loop iteration.
% %
% The difference between these atomic changes are determined via their relations with the unchanged parts. 
% %


% \textbf{Observation 3}. \textit{Changes/Transformations in code elements as well as in code structure, execution flow, and dependencies could provide rich information for understanding, determining, and inspecting vulnerabilities}. 
% %
% In Fig.~\ref{fig:fixing}, commit \texttt{4fd1e2e} removing the call of \texttt{av\_free\_packet} at line 1352, and adding the same call at line 1353 (outside the the \texttt{if} block). 
% The changes in the code structure lead to the changes in program dependencies that the call is no longer control-dependent on the \texttt{if}-statement (line 1349), and a new control dependency of the call on the \texttt{while}-statement at line 1346. 
% %
% As a result, the execution flow is also changed to that instead of only when decoding (inside the \texttt{if} block), \texttt{av\_free\_packet} is always called in the \texttt{while}-loop to free the packet data. 

% % For example, deleting a condition (if statement) makes a vulnerable statement unguarded. The changes in execution flow and dependency are vulnerable.


% \subsection{Approach Overview}
% incorporates the rich sources of information from both changed code and unchanged code.

==> [TSE'23] Just-In-Time Software Vulnerability Detection/4.ctg.tex <==
\section{Semantic Change Representation}


\subsection{Relational Code Graph}
From our point of view, a program is a set of \textit{inter-related elements} and \textit{relations} with other entities. 
%
Essentially, both the syntactic and semantic aspects of programs are necessary to properly understand the program~\cite{joern, ngo2021ranking}. 
% In the literature, the semantics of programs could be captured well via the \textit{structure} and \textit{dependency} relations in graphs.
%
% In this work, we use a graph-based representation that connects code elements in  \textit{structure} and \textit{dependency} relations to represent the program. Specially, the structure relations represent the syntax of the program, meanwhile, its semantics are captured by the dependency relations.
In this work, we use a graph-based representation, \textit{Relational Code Graph}, for programs that represents the code elements as well as the syntactic aspect 
% the programs
via the \textit{structure} relation and the semantic aspect via the \textit{dependency} relation.
%
%  


\begin{definition}[Relational Code Graph]
For a code snippet $f$, the corresponding relational code graph, a directed graph $G_f = \langle N, E, \mathcal{R} \rangle$, represents the structure and dependencies of $f$. Formally, $G_f = \langle N, E, \mathcal{R} \rangle$ is defined as followings:
\begin{itemize}
    \item $N$ is a set of nodes which are the AST nodes of $f$. In $N$, the leaf nodes are code tokens, while internal (non-leaf) nodes are abstract syntactic code elements (e.g., statements, predicate expressions, assignments, or function calls).
    
    \item $E$ is a set of edges that represent certain relations between nodes, such relations are either structure or dependency. For $n_i, n_j \in N$, an edge exists from $n_i$ to $n_j$ regarding relation $r \in \mathcal{R} = \{\textit{structure, dependency}\}$, $\exists e^r_{ij} = \langle n_i, r, n_j \rangle \in E$ if there is a relation $r$ between $n_i$ and $n_j$. 
    
\end{itemize}
\end{definition}
%
Note that the dependency edges connect the nodes which are statements or predicate expressions~\cite{pdg}. Each statement/predicate expression contains the descendants which are connected via the structure edges.
%
The reason for the incorporation of multiple kinds of knowledge about code in a single representation instead of using multiple graphs is that structural information could explain the dependencies between nodes.
%
%
For example, Fig.~\ref{fig:before-after} shows the relational code graphs of the function before and after the change in Fig.~\ref{fig:example_change}.
%
Statement $s$ at line 3 of Fig.~\ref{fig:example_change} assigns ($=$) a value to variable \texttt{len} which is used by statement $s'$ at line 4. There is a data-dependency relation from the statement node corresponding to $s$ to the statement node corresponding to $s'$ (Fig.~\ref{fig:before-after}).
Explicitly representing the structures of $s$ (variable \texttt{len}, assignment operator, and \texttt{strlen(str)}) and $s'$ (\texttt{len} as an argument of \texttt{memcpy}) could help explain the existence of the dependency edge from $s$ to $s'$.
%
%
%
In this work, we use Joern analyzer~\cite{joern} as a tool to analyze code and determine the structure and dependency relations between code elements to construct relational code graphs. 
% In general, ones could consider the relations between the nodes other than the structure and dependency such as control-flow or data-flow. 
%


\begin{figure}
    \centering
    \includegraphics[width=0.7\columnwidth]{imgs/example_BO.png}
    \caption{A dangerous commit causing a \textit{Buffer Overflow} vulnerability}
    \label{fig:example_change}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1.0\columnwidth]{imgs/before-after.png}
    \caption{The relational code graphs before and after the change in Fig.~\ref{fig:example_change}}
    \label{fig:before-after}
\end{figure}


\subsection{Code Transformation Graph}
\label{sec:ctg}


% In this work, we aim to represent the code changes of commits using graphs which can capture the code structure and semantics as well as the code transformations caused by the changes. 
In this work, we aim to represent the code transformations by commits in both the code structure and the dependencies using graphs. 
%
As explained in Sec.~\ref{sec:example}, the changes should be represented in the context of the unchanged parts, as well as the transformations in the code elements and the relations between the elements. 

\begin{definition}[Code Transformation Graph (CTG)]
For a commit changing code from a version 
% ($o$) 
to another, 
% ($n$),
the \textit{code transformation graph} is an annotated graph constructed from the relational code graphs of these two versions. Formally, for $G_o = \langle N_o, E_o, \mathcal{R} \rangle$ and $G_{n} = \langle N_n, E_n, \mathcal{R} \rangle$ which are the relational code graphs of the old version and the new version respectively, the CTG $\mathcal{G} = \langle \mathcal{N}, \mathcal{E}, \mathcal{R}, \alpha \rangle$ is defined as followings:
\begin{itemize}
    \item $\mathcal{N}$ consists of the code elements in the changed and unchanged parts, $\mathcal{N} = N_o \cup N_n$.
    %
    
    \item $\mathcal{E}$ is the set of the edges representing the relations between nodes, $\mathcal{E} = E_o \cup E_n$.

    \item $\mathcal{R}$ is a set of the considered relations between code elements, $\mathcal{R} = \{\textit{structure, dependency}\}$.
    
    \item Annotations for nodes and edges are either \textit{unchanged}, \textit{added}, or \textit{deleted} by the change. Formally, $\alpha(g) \in \{$\textit{unchanged}, \textit{added}, \textit{deleted}$\}$, where $g$ is a node in $\mathcal{N}$ or an edge in $\mathcal{E}$:
        \begin{itemize}
            \item $\alpha(g) =$ \textit{added} if $g$ is a node and $g \in N_n \setminus N_o$, or $g$ is an edge and $g \in E_n \setminus E_o$
            \item $\alpha(g) =$ \textit{deleted} if $g$ is a node and $g \in N_o \setminus N_n$, or $g$ is an edge and $g \in E_o \setminus E_n$
            \item Otherwise, $\alpha(g) = $ \textit{unchanged} 
        \end{itemize}
\end{itemize}
\end{definition}


The CTG of the change in Fig.~\ref{fig:example_change} is partially shown in Fig.~\ref{fig:example_ctg}. As we could see the structure changes, the structure of the predicate expression at line 4 is changed. Specifically, \texttt{2*BUF\_SIZE} is replaced by \texttt{BUF\_SIZE} in the right-hand side of the less-than comparison expression. This allows the statement at line 5 to be executed even when \texttt{len > BUF\_SIZE}. In the CTG, through PDG edges, the statement copies \texttt{len} (defined at line 3) bytes from \texttt{str} (declared at line 1) to \texttt{buf} (declared at line 2) which can have maximum \texttt{BUF\_SIZE} bytes or even greater. This will cause an overflow error when \texttt{2*BUF\_SIZE > len > BUF\_SIZE}.


Theoretically, a CTG corresponding to a commit could be very large and contain many unchanged nodes/edges which are irrelevant to the changes. These irrelevant parts might be unnecessary to capture the changes' meaning and also produce noise for understanding the changes. To trim those irrelevant parts, the nodes/edges that are not relevant to the changed nodes/edges are removed from $\mathcal{G}$. 
%
Our idea is that all the statements/predicate expressions containing changed nodes and their related statements/expressions via dependencies are kept. Additionally, the descendant nodes of these statements/expressions are also retained in the graph to enable further elaboration.
%
Formally, given CTG $\mathcal{G} = \langle \mathcal{N}, \mathcal{E}, \mathcal{R}, \alpha \rangle$, a node $n$ is considered as \textit{relevant} to the change if $n$ satisfies one of the following conditions:
%
\begin{itemize}
    % \item $n$ is a statement/predicate expression node, $n$ is deleted/added (i.e., $\alpha(n) \neq $ \textit{unchanged}).
    
    \item $n$ is a statement/predicate expression node which is the ancestor of a deleted/added node $n'$. In other words, there is a path from $n$ to $n'$ only via structure- edges.
    
    \item $n$ is a statement/predicate expression node, and $n$ impact/is impacted by a \textit{relevant} node $n'$. In other words, there is a path from $n$ to $n'$ or from $n'$ to $n$ via dependency edges.

    \item $n$ is a descendant of a relevant node $n'$. In other words, there is a path from $n'$ to $n$ only via structure edges.
    
\end{itemize}
%
After trimming, the simplified CTG contains the nodes which are relevant to the changes. The edges which do not connect any pair of nodes are also removed from the graph.
 

\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{imgs/ctg.png}
    \caption{The CTG corresponding to the change in Fig.~\ref{fig:example_change}}
    \label{fig:example_ctg}
\end{figure}




==> [TSE'23] Just-In-Time Software Vulnerability Detection/5.framework.tex <==
\section{Code-centric Just-In-Time Vulnerability Detection with Graph Neural Networks}





Fig.~\ref{fig:model} shows the overview of our JIT-VD model. In this work, each CTG is treated as a relational graph. 
%
% Additionally, to form  programs' behaviors, the nodes interact with each others via their relations. 
%
% Additionally, besides the nodes of CTGs, the 
%
To capture the important features of the graphs, not only the contents of the nodes but also their relations need to be considered in JIT-VD. 
For this purpose, we apply relational graph neural networks~\cite{rgat, rgcn} for the JIT-VD task.
%
% The model extracts the features to represent the nodes and edges in the constructed CTGs of the known commits. 



First, the nodes are embedded into $d$-dimensional hidden features $n_i$ produced by embedding the content of the nodes. 
%
Particularly, to build the vectors for nodes' content, we use Word2vec~\cite{word2vec_1} which is widely used to capture semantic similarity among code tokens~\cite{embedding_emse22}.
%
%
%
Then, to form the node feature vectors, the node embedding vectors are annotated with the change operators (\textit{added}, \textit{deleted}, and \textit{unchanged}) by concatenating corresponding one-hot vector of the operators to the embedded vectors, $h^{0}_i = n_i \bigoplus \alpha(n_i)$, where $\bigoplus$ is the concatenating operator and $\alpha$ returns the one-hot vector corresponding the annotation of node $i$.
%
%
The resulting vectors are fed to a relational graph neural network model which could be a relational graph convolution network (RGCN)~\cite{rgcn} or a relational graph attention (RGAT) model~\cite{rgat}.
%
%
Each layer of RGCN or RGAT computes the representations for the nodes of the graph through message passing, where each node gathers features from its neighbors under every relation to represent the local graph structure. Stacking $L$ layers allows the network to build node representations from the $L$-hop neighborhood of each node.
% This guarantees the transformation to build local reception fields and be invariant to both graph size and vertex re-indexing.
%
%
Thus, the feature vector $h^{l+1}_{i}$ at node $i$ at the next layer is: 
%
\begin{equation} \label{eq:propagate_rule}
h^{l+1}_{i} =\sigma \left( 
\sum_{r \in \mathcal{R}}
    \sum_{j \in \mathcal{N}^r_i} \frac{1}{c_{i,r}} g_j^r
\right)
\end{equation}
%
%
%
%
% h^{l+1}_{i} =\sigma \left( \sum_{j \in \mathcal{N}_i} \frac{1}{c_{ij}} h^{l}_{i} W^l \right)
%
% h^{l+1}_{i} =\sigma \left( 
% W^l_0 h^{l}_{i} + 
% \sum_{r \in \mathcal{R}}
%     \sum_{j \in \mathcal{N}^r_i} \frac{1}{c_{i,r}}  W^l_r h^{l}_{j} 
% \right)
%
%
%
where $g_j = W^l_r h^{l}_{j}$ is the distinct intermediate representation of node $j$ under relation $r$, $W^l_r$ is a learnable weight matrix for feature transformation specific for relation $r$. In equation (\ref{eq:propagate_rule}), $\mathcal{N}^r_i$ is the set of neighbor indices of node $i$ under relation $r \in \mathcal{R} = \{\textit{structure, dependency}\}$.
% including \textit{structure}, \textit{execution flow}, \textit{dependency}, and \textit{self-connection} which is a single special relation from node $i$ to itself.
%
Additionally, $1/c_{i}^r$ is a problem-specific normalization constant that can be chosen in advance (such as $c_{i}^r = |\mathcal{N}_i^r|$). 
%
% $c_{ij} =\sqrt{|\mathcal{N}_i| \times |\mathcal{N}_j|}$ is a normalization constant based on graph structure, 
Meanwhile, $\sigma$ is a non-linear activation function such as ReLU.
%
In this work, instead of using constant $1/c_{i}^r = |\mathcal{N}_i^r|^{-1}$, we replace the normalization constant by an learnable attention weight $a_{ij}^r$, where $\sum_{j,r} a_{ij}^r = 1$, to allow the model learn the importance of node $j$ and the relation between node $i$ and node $j$ under relation $r$~\cite{rgat}:
%
% Particularly, 
%
$$
a_{ij}^r = \text{softmax}_{j}(E_{ij}^r) =  \frac{\exp{(E_{ij}^r)}}{\sum_{k \in \mathcal{N}^r_i} \exp{(E_{ik}^r)}} 
$$
%
%
$$
E_{ij}^r = \text{LeakyReLu}(q_i^r + k_j^r)
$$
%
$$
q_i^r = g_i^r Q^r, \text{ and } k_j^r = g_j^r K^r
$$
%
%
where $Q^r$ and $K^r$ are the query kernel and key kernel projecting $g_i$ (and $g_j$) into query and key representations~\cite{rgat}. $Q^r$ and $K^r$ are combined to form the attention kernel for relation $r$, $A^r = Q^r \bigoplus K^r$.

% After $L$ RGAT layers, a $d$-dimensional graph-level vector representation $H$ for the whole CTG $\mathcal{G} = \langle \mathcal{N}, \mathcal{E}, \alpha \rangle$ is built by averaging over all node features in the final RGAT layer, $H = \frac{1}{|\mathcal{N}|} \sum_{i \in [1, |\mathcal{N}|]} h^L_i$.
%
After $L$ GNN layers, a $d$-dimensional graph-level vector representation $H$ for the whole CTG $\mathcal{G} = \langle \mathcal{N}, \mathcal{E}, \alpha \rangle$ is built by aggregating over all node features in the final GNN layer, $H = \Phi_{i \in [1, |\mathcal{N}|]} h^L_i$, where $\Phi$ is a graph readout function such as \textit{sum}, \textit{average}, or \textit{max}. The impact of the aggregation function $\Phi$ on \tool's performance will be empirically shown in Sec.~\ref{sec:results}.
%
%
Finally, the graph features are then passed to a Multilayer perceptron (MLP) to classify if $\mathcal{G}$ is dangerous or not.

\begin{figure*}
    \centering
    \includegraphics[width=2.0\columnwidth]{imgs/model.png}
    \caption{Just-In-Time Vulnerability Detection Model in \tool}
    \label{fig:model}
\end{figure*}














% Figure~\ref{fig:framework} shows the overview of our integrated code-centric framework for detecting and localizing \jit vulnerabilities. There are three phases in our framework: \textit{training}, \textit{inferring}, and \textit{inspecting}. 
% %
% First, each commit and the containing repository in this framework will be used to construct its CTG. 
% %
% In the \textit{training} phase, the constructed CTGs of the previously known dangerous/clean commits are fed to a classification model (JIT-VD model) and learn how to discriminate between dangerous and safe commits. 
% %
% In the \textit{inferring} phase, given a commit, the trained JIT-VD model determines if the commit is suspicious or not using its CTG. 
% %
% Then, for each predicted suspicious commit, the \textit{interpreting} phase utilizes the insights in the decision-making process of the JIT-VD model for identifying the suspicious code.
% Particularly, the model and its prediction of the input CTG are interpreted to determine the code elements important for the models' decision. These elements are refined to identify suspicious statements. If the model determines the commit as safe, then this phase can also point out the key elements that are deemed to be safe.


% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\columnwidth]{imgs/framework.png}
%     \caption{Integrated code-centric JIT vulnerability detection \& inspection framework}
%     \label{fig:framework}
% \end{figure}


% \input{5.framework/5.1.vul_detection.tex}

% \input{5.framework/5.2.vul_inspection.tex}




































































%SON OLD
% First, nodes and edges are embedded into $d$-dimensional hidden features $h_i$ and $e_{ij}$ produced by embedding the content of the nodes and edges.
% %
% Then, the node embedding vectors and and edge embedding vectors are annotated the change operators (\textit{added}, \textit{deleted}, and \textit{remained}) by concatenating the encoded vectors of the change operators to the embedded vectors, $h^{0}_i=concat(h^{0}_i, cop[h^{0}_i])$ and $e^{0}_{ij}=concat(e^{0}_{ij}, cop[e^{0}_{ij}])$.
% %
% %
% The resulting vectors are fed to a graph neural network (GNN) model. In this work, we treat each CTG as a renational heterogeneous graph, and use relational graph convolution network (R-GCN)~\cite{r-gnn} to classify the CTGs of commits. 
% %
% %
% In GCNs, each layer computes the representations for the nodes of the graph through message passing, where each node gathers features from its neighbors under every relation to represent local graph structure~\cite{?}. Stacking $L$ layers allows the network to build node representations from the $L$-hop neighborhood of each node.
% % This guarantees the transformation to build local reception fields and be invariant to both graph size and vertex re-indexing.
% %
% %
% Thus, the feature vector $h^{l+1}_{i}$ at node $i$ at the next layer in the R-GNN is: 
% %
% $$
% % h^{l+1}_{i} =\sigma \left( \sum_{j \in \mathcal{N}_i} \frac{1}{c_{ij}} h^{l}_{i} W^l \right)
% %
% h^{l+1}_{i} =\sigma \left( 
% W^l_0 h^{l}_{i} + 
% \sum_{r \in \mathcal{R}}
%     \sum_{j \in \mathcal{N}^r_i} \frac{1}{c_{i,r}}  W^l_r h^{l}_{j} 
% \right)
% %
% $$
% %
% where $\mathcal{N}^r_i$ is the set of neighbor indices of node $i$ under relation $r \in \mathcal{R} = \{\text{structure}, \text{execution flow}, \text{dependency}\}$, $c_{i,r}$ is a problem-specific normalization constant that can be chosen in advance (such as $c_{i,r} = |\mathcal{N}_i^r|$). 
% %
% $W^l_r$ is a learnable weight matrix for feature transformation specific for relation $r$, while $W^l_0$ is a linear projection via a learnable weight matrix for a single self-connection of a special relation
% type to node $i$,
% % $c_{ij} =\sqrt{|\mathcal{N}_i| \times |\mathcal{N}_j|}$ is a normalization constant based on graph structure, 
% and $\sigma$ is an non-linear activation function such as ReLU.
% %
% In this work, instead of using $1/c_{i,r}$ which is a constant, we replace by an learnable attention weight $a_{ij,r}$, where $\sum_{j,r} a_{ij,r} = 1$, to allow the model learn the importance of node $j$ and the relation between node $i$ and node $j$ under relation $r$~\cite{gat}. 
% %
% % Particularly, 
% % %
% % $$
% % \alpha_{ij,r} = softmax_{j,r}(e_{ij,r}) =  \frac{\exp{(e_{ij,r})}}{\sum_{j \in \mathcal{N}^r_i} \exp{(e_{ik,r})}} 
% % % \frac{\exp{e_{ij,r}}{}
% % % \sum_{j \in \mathcal{N}^r_i} \exp{e_{ik,r}}
% % $$
% %
% After $L$ R-GNN layers, a $d$-dimensional graph-level vector representation $X_\mathcal{G}$ for the whole CTG $\mathcal{G} = \langle \mathcal{N}, \mathcal{E}, \alpha \rangle$ is built by averaging over all node features in the final R-GCN layer, $X_\mathcal{G} = \frac{1}{|\mathcal{N}|} \sum_{i \in [0, |\mathcal{N}|]} h^L_i$. Finally, the graph features are then passed to a Multilayer perceptron (MLP) to classify if $\mathcal{G}$ is dangerous or not.

% \begin{figure*}
%     \centering
%     \includegraphics[width=2.0\columnwidth]{imgs/model.png}
%     \caption{Just-In-Time Vulnerability Detection Model}
%     \label{fig:model}
% \end{figure*}

==> [TSE'23] Just-In-Time Software Vulnerability Detection/5.framework/5.1.vul_detection.tex <==
\subsection{Code-centric Just-In-Time Vulnerability Detection}
Fig.~\ref{fig:model} shows our JIT-VD model. In this work, we treat each CTG as a relational heterogeneous graph and thus apply relational graph attention networks~\cite{rgat} for the JIT-VD task.
%
% The model extracts the features to represent the nodes and edges in the constructed CTGs of the known commits. 



First, the nodes are embedded into $d$-dimensional hidden features $n_i$ produced by embedding the content of the nodes.
%
Then, to form the node feature vectors, the node embedding vectors are annotated the change operators (\textit{added}, \textit{deleted}, and \textit{remained}) by concatenating corresponding one-hot vector of the operators to the embedded vectors, $h^{0}_i = n_i \bigoplus \alpha(n_i)$, where $\bigoplus$ is the concatenating operator and $\alpha$ returns the one-hot vector corresponding the annotation of node $i$.
%
%
The resulting vectors are fed to a relational graph attention (RGAT) model.
%
%
Similar to general relational graph convolution network (RGCN)~\cite{rgcn}, each layer of RGAT computes the representations for the nodes of the graph through message passing, where each node gathers features from its neighbors under every relation to represent local graph structure. Stacking $L$ layers allows the network to build node representations from the $L$-hop neighborhood of each node.
% This guarantees the transformation to build local reception fields and be invariant to both graph size and vertex re-indexing.
%
%
Thus, the feature vector $h^{l+1}_{i}$ at node $i$ at the next layer in RGAT is: 
%
\begin{equation} \label{eq:propagate_rule}
h^{l+1}_{i} =\sigma \left( 
\sum_{r \in \mathcal{R}}
    \sum_{j \in \mathcal{N}^r_i} \frac{1}{c_{i,r}} g_j^r
\right)
\end{equation}
%
%
%
%
% h^{l+1}_{i} =\sigma \left( \sum_{j \in \mathcal{N}_i} \frac{1}{c_{ij}} h^{l}_{i} W^l \right)
%
% h^{l+1}_{i} =\sigma \left( 
% W^l_0 h^{l}_{i} + 
% \sum_{r \in \mathcal{R}}
%     \sum_{j \in \mathcal{N}^r_i} \frac{1}{c_{i,r}}  W^l_r h^{l}_{j} 
% \right)
%
%
%
where $g_j = W^l_r h^{l}_{j}$ is the distinct intermediate representation of node $j$ under relation $r$, $W^l_r$ is a learnable weight matrix for feature transformation specific for relation $r$. In Equation (\ref{eq:propagate_rule}), $\mathcal{N}^r_i$ is the set of neighbor indices of node $i$ under relation $r \in \mathcal{R}$.
% including \textit{structure}, \textit{execution flow}, \textit{dependency}, and \textit{self-connection} which is a single special relation from node $i$ to itself.
%
Additionally, $1/c_{i}^r$ is a problem-specific normalization constant that can be chosen in advance (such as $c_{i}^r = |\mathcal{N}_i^r|$). 
%
% $c_{ij} =\sqrt{|\mathcal{N}_i| \times |\mathcal{N}_j|}$ is a normalization constant based on graph structure, 
Meanwhile, $\sigma$ is a non-linear activation function such as ReLU.
%
In this work, instead of using constant $1/c_{i}^r = |\mathcal{N}_i^r|^{-1}$, we replace the normalization constant by an learnable attention weight $a_{ij}^r$, where $\sum_{j,r} a_{ij}^r = 1$, to allow the model learn the importance of node $j$ and the relation between node $i$ and node $j$ under relation $r$~\cite{rgat}:
%
% Particularly, 
%
$$
a_{ij}^r = \text{softmax}_{j}(E_{ij}^r) =  \frac{\exp{(E_{ij}^r)}}{\sum_{k \in \mathcal{N}^r_i} \exp{(E_{ik}^r)}} 
$$
%
%
$$
E_{ij}^r = \text{LeakyReLu}(q_i^r + k_j^r)
$$
%
$$
q_i^r = g_i^r Q^r, \text{ and } k_j^r = g_j^r K^r
$$
%
%
where $Q^r$ and $K^r$ are the query kernel and key kernel projecting $g_i$ (and $g_j$) into query and key representations~\cite{rgat}. $Q^r$ and $K^r$ are combined to form the attention kernel for relation $r$, $A^r = Q^r \bigoplus K^r$.

After $L$ RGAT layers, a $d$-dimensional graph-level vector representation $H$ for the whole CTG $\mathcal{G} = \langle \mathcal{N}, \mathcal{E}, \alpha \rangle$ is built by averaging over all node features in the final RGAT layer, $H = \frac{1}{|\mathcal{N}|} \sum_{i \in [1, |\mathcal{N}|]} h^L_i$. Finally, the graph features are then passed to a Multilayer perceptron (MLP) to classify if $\mathcal{G}$ is dangerous or not.

\begin{figure*}
    \centering
    \includegraphics[width=2.0\columnwidth]{imgs/model.png}
    \caption{Just-In-Time Vulnerability Detection Model}
    \label{fig:model}
\end{figure*}



















































































%SON OLD
% First, nodes and edges are embedded into $d$-dimensional hidden features $h_i$ and $e_{ij}$ produced by embedding the content of the nodes and edges.
% %
% Then, the node embedding vectors and and edge embedding vectors are annotated the change operators (\textit{added}, \textit{deleted}, and \textit{remained}) by concatenating the encoded vectors of the change operators to the embedded vectors, $h^{0}_i=concat(h^{0}_i, cop[h^{0}_i])$ and $e^{0}_{ij}=concat(e^{0}_{ij}, cop[e^{0}_{ij}])$.
% %
% %
% The resulting vectors are fed to a graph neural network (GNN) model. In this work, we treat each CTG as a renational heterogeneous graph, and use relational graph convolution network (R-GCN)~\cite{r-gnn} to classify the CTGs of commits. 
% %
% %
% In GCNs, each layer computes the representations for the nodes of the graph through message passing, where each node gathers features from its neighbors under every relation to represent local graph structure~\cite{?}. Stacking $L$ layers allows the network to build node representations from the $L$-hop neighborhood of each node.
% % This guarantees the transformation to build local reception fields and be invariant to both graph size and vertex re-indexing.
% %
% %
% Thus, the feature vector $h^{l+1}_{i}$ at node $i$ at the next layer in the R-GNN is: 
% %
% $$
% % h^{l+1}_{i} =\sigma \left( \sum_{j \in \mathcal{N}_i} \frac{1}{c_{ij}} h^{l}_{i} W^l \right)
% %
% h^{l+1}_{i} =\sigma \left( 
% W^l_0 h^{l}_{i} + 
% \sum_{r \in \mathcal{R}}
%     \sum_{j \in \mathcal{N}^r_i} \frac{1}{c_{i,r}}  W^l_r h^{l}_{j} 
% \right)
% %
% $$
% %
% where $\mathcal{N}^r_i$ is the set of neighbor indices of node $i$ under relation $r \in \mathcal{R} = \{\text{structure}, \text{execution flow}, \text{dependency}\}$, $c_{i,r}$ is a problem-specific normalization constant that can be chosen in advance (such as $c_{i,r} = |\mathcal{N}_i^r|$). 
% %
% $W^l_r$ is a learnable weight matrix for feature transformation specific for relation $r$, while $W^l_0$ is a linear projection via a learnable weight matrix for a single self-connection of a special relation
% type to node $i$,
% % $c_{ij} =\sqrt{|\mathcal{N}_i| \times |\mathcal{N}_j|}$ is a normalization constant based on graph structure, 
% and $\sigma$ is an non-linear activation function such as ReLU.
% %
% In this work, instead of using $1/c_{i,r}$ which is a constant, we replace by an learnable attention weight $a_{ij,r}$, where $\sum_{j,r} a_{ij,r} = 1$, to allow the model learn the importance of node $j$ and the relation between node $i$ and node $j$ under relation $r$~\cite{gat}. 
% %
% % Particularly, 
% % %
% % $$
% % \alpha_{ij,r} = softmax_{j,r}(e_{ij,r}) =  \frac{\exp{(e_{ij,r})}}{\sum_{j \in \mathcal{N}^r_i} \exp{(e_{ik,r})}} 
% % % \frac{\exp{e_{ij,r}}{}
% % % \sum_{j \in \mathcal{N}^r_i} \exp{e_{ik,r}}
% % $$
% %
% After $L$ R-GNN layers, a $d$-dimensional graph-level vector representation $X_\mathcal{G}$ for the whole CTG $\mathcal{G} = \langle \mathcal{N}, \mathcal{E}, \alpha \rangle$ is built by averaging over all node features in the final R-GCN layer, $X_\mathcal{G} = \frac{1}{|\mathcal{N}|} \sum_{i \in [0, |\mathcal{N}|]} h^L_i$. Finally, the graph features are then passed to a Multilayer perceptron (MLP) to classify if $\mathcal{G}$ is dangerous or not.

% \begin{figure*}
%     \centering
%     \includegraphics[width=2.0\columnwidth]{imgs/model.png}
%     \caption{Just-In-Time Vulnerability Detection Model}
%     \label{fig:model}
% \end{figure*}

==> [TSE'23] Just-In-Time Software Vulnerability Detection/5.framework/5.2.vul_inspection.tex <==
\subsection{Integrated Just-In-Time Vulnerability Localization}
After a suspicious commit is detected by our JIT-VD model, to utilizing the insights from the model's decision-making process for narrowing down the search space for the dangerous changes, a model interpreter is employed to provide the explanations of the model's decision. The explanations should point down which parts (nodes and edges) in the CTG are the deciding elements for the model's conclusion. These important edges/nodes are use to identify the (un)changed code statements in the commit which suspiciously cause vulnerabilities in the code.
%
%

For a trained JIT-VD model and its prediction for a CTG $\mathcal{G} = \langle \mathcal{N}, \mathcal{E}, \mathcal{R}, \alpha \rangle$, an interpreter assigns an importance score to either each edge $e^r_{ij} \in \mathcal{E}$ or each node $n_i \in \mathcal{N}$ by the edge importance function or the node importance function. Formally, $\textit{IM}_\mathcal{N}: \mathcal{N} \to [0,1]$ and  $\textit{IM}_\mathcal{E}: \mathcal{E} \to [0,1]$, the higher $\textit{IM}_\mathcal{E}(e^r_{ij})$ and $\textit{IM}_\mathcal{N}(n_i)$, the more important edge $e$ and node $n$ to the model's prediction for $\mathcal{G}$.
%
%
%
Intuitively, a statement in $\mathcal{G}$ contains more important elements, then the statement is more suspicious. Thus, given the node importance function $\textit{IM}_\mathcal{N}$, the suspiciousness of a statement node, $s \in \mathcal{N}$ corresponding to a code statement is determined by summing the importance scores of all the AST descendants of $s$:
%
%
\begin{equation} \label{eq:suspiciousness}
% \mathscr{S}(s) = \max_{n \in \textit{Desc}(s)} \textit{IM}_\mathcal{N}(n)
\mathscr{S}(s) = \sum_{n \in \textit{Desc}(s)} \textit{IM}_\mathcal{N}(n)
\end{equation}
%
%
where $\textit{Desc}(s) \subset \mathcal{N}$ returns the set of AST descendant nodes of $s$, which can be collected by traversing $\mathcal{G}$ from $s$ on structure edges. Meanwhile, if the edge importance function $\textit{IM}_\mathcal{E}$ is provided instead of the node importance function, we derive the importance of a node $n \in \mathcal{N}$ as: 
%
%
\begin{equation} \label{eq:importance_node}
\textit{IM}_\mathcal{N}(n_i) = \max_{r \in \mathcal{R}} 
\left( 
\sum_{j \in \mathcal{N}^r_i} \textit{IM}_\mathcal{E}(e^r_{ij})
+
\sum_{k \in \mathcal{N}^{-r}_i} \textit{IM}_\mathcal{E}(e^r_{ki})
\right)
\end{equation}
%
%
where $\mathcal{N}^r_i$ is the set of neighbor indices of $n_i$ under relation $r \in \mathcal{R}$, while $\forall k \in \mathcal{N}^{-r}_i$, there is an edge $\langle n_i, r, n_k \rangle \in \mathcal{E}$. The intuition of (\ref{eq:importance_node}) is that $n_i$ is more important regarding a relation $r \in \mathcal{R}$ if there are more important $r$-edges directly relevant to $n_i$. The overall importance of $n_i$ is the highest importance score among the scores regarding all relations.


% This could be done by the perturbation-based GNN explanation techniques which is widely employed to explain GNN models. These techniques assume that important input parts significantly contribute to the decisions while unimportant parts have minor influences. Based on the model and its decision, these methods score the importance of the input parts.
%
%

% To derive explanations, the general goal of perturbation-based methods is to reduce redundant information in a graph which does not directly impact the model's decisions. For a CTG $\mathcal{G}$, the approaches find the compact sub-graph $\mathcal{G_S}$ of $\mathcal{G}$ that minimizes the deference in the prediction scores using $\mathcal{G}$ and $\mathcal{G_S}$. 
%
% This task is treated as generating a mask for edges/nodes/node features to explain the predictions via mask optimization. The masks are obtained in different methods with various objective functions to indicate the input importance. The generated masks are combined with $\mathcal{G}$ to obtain $\mathcal{G_S}$ containing important input information.
%
% Finally, $\mathcal{G_S}$ is fed into the trained JIT-VD model to evaluate the masks and update the mask generation methods.
%
% Intuitively, the masks should capture the important parts which convey the key semantic meaning of $\mathcal{G}$, and hence the model produces a similar prediction to the prediction for $\mathcal{G}$. 
%
%

In general, any GNN explanation technique e.g., GNNExplainer~\cite{gnn_explainer} or AttentionExplainer could be applied to provide $\textit{IM}_\mathcal{N}$ or $\textit{IM}_\mathcal{E}$.
%
% In this work, we apply GNNExplainer~\cite{gnn_explainer} which is a popular perturbation-based technique for the model explanation step in our framework. The masks are optimized by maximizing the mutual information between the predictions of $\mathcal{G}$ and the predictions of the newly obtained graph~\cite{gnn_explainer}.
%
The impact of selecting the explanation technique in our framework on vulnerability localization performance will be empirically shown in Section~\ref{sec:intrinsic}. 




% The resulting sub-graph $\mathcal{G_S}$ is directly used as an interpretation. We can similarly produce the interpretations for the cases of non-vulnerability result....(statement level)


% Generally, to derive explanations, the goal of perturbation-based approaches is to reduce redundant information in a graph which does not directly impact the model's decisions. For a CTG $\mathcal{G}$, the approaches find the minimal sub-graph $\mathcal{G_S}$ of $\mathcal{G}$ that minimizes the deference in the prediction scores using $\mathcal{G}$ and $\mathcal{G_S}$. Particularly, this task is treated as generating a mask for edges/nodes to explain the predictions via mask optimization. 
%
% The masks are optimized by maximizing the mutual information between the predictions of $\mathcal{G}$ and the predictions of the newly obtained graph.

==> [TSE'23] Just-In-Time Software Vulnerability Detection/6.eval_method.tex <==
\section{Evaluation Methodology}
\label{sec:eval}
To evaluate our \jit vulnerability detection approach, we seek to answer the following research questions:

\noindent\textbf{RQ1: \textit{Accuracy and Comparison}.} How accurate is {\tool} in detecting dangerous commits? And how is it compared to the state-of-the-art approaches~\cite{vccfinder,cc2vec,codereviewer}?


\noindent\textbf{RQ2: \textit{Intrinsic Analysis}.} How do the JIT-VD model's properties/components, including the GNN model, the number of GNN layers, and the graph readout function in {\tool} impact \tool's performance?

\noindent\textbf{RQ3: \textit{Change Representation Analysis}.} How do related unchanged parts in CTGs impact {\tool}'s performance? And, how do the structure relation and dependency relation in CTGs impact {\tool}'s performance?

\noindent\textbf{RQ4: \textit{Sensitivity Analysis}.} How do various the input's factors, including training data size and changed code's complexity affect {\tool}'s performance?

\noindent\textbf{RQ5: \textit{Time Complexity}.} What is  {\tool}'s running time?



\input{6.evel_method/dataset.tex}

\input{6.evel_method/method.tex}












% Our goals of the evaluation plan include 1) the evaluation of the understanding of the code characteristics of dangerous/safe commits, 2) the evaluation of detection models and techniques for potential risky/safe commits, 3) the evaluation of the quality of the vulnerability localizing/fixing guidance from our algorithms and tools, and 4) the evaluation on time and effort that our tools could save for developers in the vulnerability debugging process. 
% %
% %
% For goal 1, the correctness in the understanding of characteristics of recurring fixes will be evaluated in the performance evaluation for goals 2 and 3, in which we plan to perform empirical evaluation tasks. Finally, we plan to perform a controlled experiment for the last goal.


% \subsection{Evaluation of \jit Vulnerability Detection Model}
% We will collect data from open-source projects that provide the version history of all changes and vulnerability patches and vulnerability tracking data. We have successfully collected such data from more than 600 projects in our ongoing task (Section~\ref{sec:task_1}). We will continue our tasks with more data from open-source repositories and other sources.
% %
% Our evaluation method will include the comparison of the results produced by our tools with the oracle from human verification. The evaluation metrics could include \textit{recall}, \textit{precision}, time, and memory efficiency. Recall is the ratio between the correctly detected dangerous/safe commits over the total dangerous/safe commits existing in a project. Precision is the ratio between the correctly detected dangerous/safe commits over the total detected dangerous/safe ones.


% \subsection{Evaluation of Vulnerability Localizing/Fixing Guidance}

% We will use the same collected data as mentioned earlier. Our methodology will include the simulation of the actual vulnerability-fixing process in subject projects. For each commit that is precisely detected to be dangerous, our detection tool will recommend code elements and their relations suspiciously relevant to the causing vulnerability. Then, we will compare the recommendation locations and code elements to the actual ones in the patching commit corresponding to the dangerous commit. The primary evaluation metrics again include \textit{Rank} and \textit{Hit@X}. Rank is the average rank of actual vulnerable statements in our ranked lists. Hit@X counts the number of commits whose vulnerable statements can be found after investing $X$ ranked statements, e.g., Hit@1 counts the number of buggy statements correctly ranked 1st.


% \subsection{Evaluation on the Improvement of Developers' Effectiveness and Productivity}

% Our goal is to see how our approach improves the productivity of developers. We plan to have controlled experiments in real-world and university settings. The university setting will be the context of SE courses at Vietnam National University, Hanoi, while the real-world setting will be at our industry collaborators. We plan to have two controlled groups. Initially, they are given the same starting point of a system and required to review the same set of commits and localize vulnerable statements if they exist. One group will use our new tools while the other will not. The analyses are based on the followings (1) Controlled variables: All subjects will start from the same version and review the same set of commits. We will choose subjects with similar programming experience and provide the same training with our tools; (2) Independent variables: Using our tools or not; and (3) Dependent variables, evaluation metrics: the reviewing time and localizing vulnerability, the correct recommendations (dangerous/safe commit, etc.).



==> [TSE'23] Just-In-Time Software Vulnerability Detection/6.evel_method/dataset.tex <==
\subsection{Dataset}
\label{sec:data}
To facilitate applying advanced ML techniques to automatically and effectively learn latent and abstract dangerous commit patterns, we collected a large number of dangerous and safe commits in numerous real-world projects based on the well-known SZZ algorithm~\cite{sliwerski2005changes}. 
%
We also improved the process of collecting dangerous and safe commits in the existing work~\cite{vccfinder,vuldigger,are_we_there}.
%

% Particularly, from various vulnerability datasets~\cite{fixing_database1,bigvul,devign}, we extract the vulnerability-fixing commits.
% As these commits had already fixed problems, reviewed, and reported, it could be reasonable to consider them as \textit{safe commits}~\cite{vccfinder,are_we_there,vuldigger}. 
%
%
Particularly, to identify \textit{dangerous commits}/\textit{vulnerability contributing commits (VCCs)}~\cite{vccfinder}, the general idea is to start from vulnerable statements and identify the previous commits which last modify these statements\footnote{This can be done by using \texttt{git blame}}. 
%
Specifically, the vulnerable statements are identified from the \textit{vulnerability-fixing} commits based on the following heuristics. 
%
The statements which are deleted by the fixing commits could be considered to be vulnerable~\cite{vccfinder,vuldigger, vul_secret, bigvul}. 
%
% For the statements added by the fixing commits, the existing studies~\cite{vccfinder,vuldigger} assume that the \textit{physically} surrounding statements are vulnerable, regardless of whether these statements semantically relate to added statements or not. 
%
%
For the statements added by the fixing commits, the existing studies~\cite{vccfinder,vuldigger} assume that such statements are added to fix the nearby statements. In particular, the statements which are \textit{physically} surrounding the added statements are considered to be vulnerable regardless of whether these statements semantically relate to added statements or not. 
As a result, this procedure could miss the actual VCCs and instead blame commits which are irrelevant. To reduce this risk, we blame the statements which are \textit{semantically} related to the added statements via data/control dependencies rather than the physically surrounding ones. 

% In this work, to avoid frustrating and providing developers false-alarm warnings, we focus on vulnerability triggering commits (VTCs) which are the last VCC and expose the vulnerabilities.

% Moreover, to avoid false-positive VCCs, we focus on \textit{vulnerability triggering commits (VTCs)} which are the last commit contributing to expose the vulnerabilities. 
%
%
In practice, forming a vulnerability in a code version could require one or more VCCs over time. 
%
However, the existing studies~\cite{jit_vul_survey, fan2019impact} illustrate that various of VCCs are false positives due to refactoring operators or tangling problems of the fixing commits. For collecting VCCs, although multiple improvements of SZZ have been proposed, this is still an inevitable issue~\cite{fan2019impact}. Moreover, warning developers by providing any potential VCCs could frustrate them and make the developers spend undesirable efforts. 
%
%
%
Thus, in this work, to reduce noises while still maintaining the purpose of detecting vulnerabilities as soon as before it is merged to source code, we consider \textit{vulnerability triggering commits} as \textit{dangerous} ones which are the last VCCs triggering to fully expose vulnerabilities. 
%
%
For a commit irrelevant to a known vulnerability, it might still contain unknown vulnerabilities~\cite{vccfinder,are_we_there,vuldigger}.
Meanwhile, the fixing commits had already fixed some problems, been reviewed, and reported to the community. Thus, it could be reasonable to consider the fixing commits, which are not a VCC, as \textit{safe commits}. 


In this work, we extract the vulnerability-fixing commits from various public vulnerability datasets~\cite{fixing_database1,bigvul,devign}.
In total, we collected 20,274 commits including 11,299 safe commits and 8,975 dangerous commits from the vulnerabilities reported from Aug 1998-Aug 2022 in real-world 506 C/C++ projects such as FFmpeg, Qemu, Linux, and Tensorflow. Table~\ref{tab:dataset} shows the overview of our dataset. The details of our dataset can be found at: \textit{\url{https://github.com/ttrangnguyen/CodeJIT}}.













\begin{table}[]
\centering
\caption{Dataset statistics}
\label{tab:dataset}
\begin{tabular}{@{}lrrrr@{}}
\toprule
           & \begin{tabular}[c]{@{}r@{}}\#\textbf{Safe} \\ \textbf{commits}\end{tabular} & \begin{tabular}[c]{@{}r@{}}\#\textbf{Dangerous} \\ \textbf{commits}\end{tabular} & \textbf{\%adds} & \begin{tabular}[c]{@{}l@{}}$|N|/|E|$ \\ of \textbf{CTGs}\end{tabular} \\
           \midrule
\textit{Ffmpeg}     & 4,449 &      3,462       &     73.95               & 0.70                       \\
\textit{Qemu}     &  3,551 &      3,183       &       76.80            &  0.68                    \\
\textit{Linux}    &   783   &    780      &         78.45           &      0.66                 \\
\textit{Tensorflow} &  224   &    189       &          81.48          &  1.18                   \\
% \textit{ImageMagick}    & 71  &     76      &        59.01            &         58.99               \\
\multicolumn{5}{c}{\textit{502 projects more...}}                        \\ \midrule
\textit{Total}      &  11,299     &    8,975   &         73.31           &   0.70                     \\ \bottomrule
\end{tabular}
\end{table}


\begin{table}[]
\centering
\caption{Two evaluation settings: \dev and \cross}
\label{tab:setting-details}
\begin{tabular}{@{}clrrr@{}}
\toprule
\textbf{Setting}                        &          & \begin{tabular}[c]{@{}r@{}}\#\textbf{Dangerous} \\ \textbf{commits}\end{tabular} & \begin{tabular}[c]{@{}r@{}}\#\textbf{Safe} \\ \textbf{commits}\end{tabular} & \#\textbf{Commits} \\ \midrule
\multirow{2}{*}{\textit{Dev.-process}}  & Training & 7,748 & 8,471 & 16,219    \\
                                        & Testing  & 1,227 & 2,828 & 4,055     \\ \midrule
\multirow{2}{*}{\textit{Cross-project}} & Training & 7,714 & 9,176 & 16,890    \\
                                        & Testing  & 1,261 & 2,123 & 3,384     \\ \bottomrule
\end{tabular}
\end{table}

==> [TSE'23] Just-In-Time Software Vulnerability Detection/6.evel_method/method.tex <==
\subsection{Evaluation Setup, Procedure, and Metrics}

\subsubsection{Empirical Procedure} 

\textbf{RQ1. Accuracy and Comparison}. 

\textbf{\textit{Baselines.}} We compared \tool against the state-of-the-art JIT-VD approaches and the advanced approaches for just-in-time general defect detection adapted for JIT-VD: 

1) \textbf{VCCFinder}~\cite{vccfinder}, which uses 
commit messages and expert features to train a Support Vector Machine and is specialized for the JIT-VD task. 
%

2) \textbf{CC2Vec}~\cite{cc2vec} + \textbf{DeepJIT}~\cite{deepjit}: A CNN-based just-in-time defect prediction that the features of commits are captured by CC2Vec, a pre-trained model vectorizing commits using their changed code and commit message; 
%
%

3) \textbf{JITLine}~\cite{jitline}: A simple but effective method utilizing changed code and expert features to detect buggy commits; 
%
%

4) \textbf{LA\_Predict}~\cite{lapredict}: A regression-based approach simply using the
added-line-number feature which can outperform CC2Vec and DeepJIT; and
%
%

5) \textbf{JITFine}~\cite{jit-fine}: A DL-based approach extracting features of commits from changed code and commit message using CodeBERT as well as expert features.
%
%



\textit{\textbf{Procedure.}} In this comparative study, we evaluate the performance of the approaches in two real-world settings used in the existing studies~\cite{lapredict,jit-fine,jitline,vccfinder,cross-setting,deepjit}: \textit{development-process} and \textit{cross-project}. The details of data splitting for both settings are shown in Table~\ref{tab:setting-details}.

In the \textit{development- (dev.-) process} setting considering the impact of time on the JIT-VD approaches' performance, we follow the same time-aware evaluation procedure to construct the training data and testing data from the dataset as in the prior work~\cite{jit-fine,jitline,vccfinder,deepjit}.
Particularly, we divided the commits into those before and after time point $t$. The dangerous/safe commits before $t$ were used for training, while the commits after $t$ were used for evaluation. We selected a time point $t$ to achieve a random training/test split ratio of 80/20 based on time. Specifically, for the \textit{dev.-process} setting, the commits from Aug 1998 to Mar 2017 are used for training and the commits from Apr 2017 to Aug 2022 are for evaluation. In total, the training/test split in the number of commits for this setting is 16,219/4,055.


Similar to existing work~\cite{cross-setting,lapredict}, in the \textit{cross-project} setting, we evaluate how well the approaches can learn to recognize dangerous commits in a set of projects and detect suspicious commits in the other set. 
% This setting reflects the scenario when an approach works on a new project.
%
Specifically, the commits in a fixed set of projects are used to train the approaches, the remaining set of commits is used for testing. 
%
%
For this setting, the whole set of projects is randomly split into 80\% (402 projects) for training and 20\% (104 projects) for testing. The training/test split in the number of commits for this setting is 16,890/3,384.
%

\textbf{RQ2. Intrinsic Analysis}. We also investigated the impact of the GNN model and the number of GNN layers on \tool's JIT-VD performance. We used different variants of relational graph neural networks, and their properties to study the impact of those factors on \tool's performance.

\textbf{RQ3. Change Representation Analysis}. We studied the impacts of the code relations (structure and dependency) and unchanged code in CTGs on \tool's performance. We used different variants of CTGs and measured the performance of \tool with each variant.


\textbf{RQ4. Sensitivity Analysis}. We studied the impacts of the following factors on the performance of \tool: training size and change complexity (the rate of the changed nodes over the total of nodes in CTGs). To systematically vary these factors, we gradually added more training data, and varied the range of the change rate.

\subsubsection{Metrics}
To evaluate the JIT-VD approaches, we measure the classification \textit{accuracy}, \textit{precision}, and \textit{recall}, as well as \textit{F1} which is a harmonic mean of precision and recall. 
%
Particularly, the classification accuracy (\textit{accuracy} for short) is the fraction of the (dangerous and safe) commits which are correctly classified among all the tested commits.
%
For detecting dangerous commits, \textit{precision} is the fraction of correctly detected dangerous commits among the detected dangerous commits, while \textit{recall} is the fraction of correctly detected dangerous commits among the dangerous commits. Formally $precision = \frac{TP}{TP+FP}$ and $recall = \frac{TP}{TP+FN}$, where $TP$ is the number of true positives, $FP$ and $FN$ are the numbers of false positives and false negatives, respectively. \textit{F1} is calculated as $\textit{F1} = \frac{2 \times precision \times recall}{precision + recall}$.
%




==> [TSE'23] Just-In-Time Software Vulnerability Detection/7.results.tex <==
\section{Experimental Results}
\label{sec:results}

\input{7.results/RQ1.tex}
\input{7.results/RQ3.tex}
\input{7.results/RQ2.tex}

\input{7.results/RQ4.tex}
\input{7.results/RQ5.tex}
\input{7.results/threats.tex}


==> [TSE'23] Just-In-Time Software Vulnerability Detection/7.results/RQ1.tex <==
\subsection{JIT-VD Performance Comparison (RQ1)}
Table~\ref{tab:vd-perf-time} and Table~\ref{tab:vd-perf-proj} show the performance of \tool and the other JIT-VD approaches in the \dev and \cross settings. \tool significantly outperforms the state-of-the-art JIT-VD approaches in JIT-VD \textit{F1} and classification \textit{accuracy} in both settings. 


\input{tables/tab-jit-vd-comparison.tex}


%
In the \dev setting, the JIT-VD \textit{F1} and \textit{accuracy} of \tool are significantly better than those of the baseline approaches by \textbf{10--68\%} and \textbf{8--73\%}, respectively. Meanwhile, \tool's \textit{recall} in the \dev setting is just slightly lower than those of VCCFinder~\cite{vccfinder} and JITFine~\cite{jit-fine}, by up to 7\%. The predictions of \tool are much more precise than those of all the studied methods. Specifically, \tool improves the \textit{precision} of the other approaches by \textbf{15--136\%} in this setting.



In the \cross setting, \tool consistently improves the state-of-the-art JIT-VD approaches by \textbf{23--65}\% in JIT-VD \textit{F1} and \textbf{17--77}\% in classification \textit{accuracy}.
%
\tool achieves the \textit{recall} of \textbf{0.8}, which is significantly better than the corresponding rates achieved by all the other approaches, with improvements ranging from \textbf{11--66\%}. This means that \tool can effectively detect \textbf{8/10} dangerous commits.
%
Especially, the \textit{precision} of \tool in this setting is \textbf{90\%}. In other words, \textbf{9/10} suspicious commits detected by \tool actually are dangerous ones. Meanwhile, the corresponding figures of the existing methods are 4.0--6.8. 


Moreover, the results in Table~\ref{tab:vd-perf-time} and Table~\ref{tab:vd-perf-proj} show that \tool performs stably in both settings. Particularly, \tool consistently achieves the highest overall performance (\textit{F1} and \textit{accuracy}) among the JIT-VD approaches. \tool also maintains the same pattern of improvement for both \textit{precision} and \textit{recall} when switching between the \dev setting and \cross setting. 
%TODO: Check this one
% In other words, \tool does not sacrifice neither its \textit{precision} nor its \textit{recall} to achieve the best performance.
For most of the other approaches, an increase in \textit{precision} is typically accompanied by a decrease in \textit{recall} when switching from one setting to the other. For example, in the \dev setting, VCCFinder can find much more dangerous commits (higher \textit{recall}), yet raise more false alarms (lower \textit{precision}) compared to this approach in the \cross setting. In other words, these approaches cannot detect dangerous commit more effectively and more precisely at the same time. 




% \begin{gtheorem}
% \textbf{Answer for RQ1}: For both settings, \tool can detect not only more precisely but also more dangerous commits compared to the state-of-the-art approaches. This confirms our code-centric strategy in detecting vulnerabilities at the commit-level. 
% \end{gtheorem}

\begin{gtheorem}
\textbf{Answer for RQ1}: For both settings, \tool can precisely detect a larger number of dangerous commits compared to the state-of-the-art approaches. This confirms our code-centric strategy in detecting vulnerabilities at the commit-level. 
\end{gtheorem}



\textbf{Result Analysis.} 
%
%
%
% Fig.~\ref{fig:change_rate} show \tool's JIT-VD performance by the changed node rate of CTGs. For a CTG $\mathcal{G} = \langle \mathcal{N}, \mathcal{E}, \mathcal{R}, \alpha \rangle$, the changed node rate is calculated as $\frac{|C|}{|\mathcal{N}|}$, where $C$ is the set of nodes whose annotation is not \textit{unchanged}. The rate could reflect the complexity of the code changes.
%
%
% As seen, the more complex change 
%
% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\columnwidth]{imgs/change_rate.png}
%     \caption{Performance by changed node rates}
%     \label{fig:change_rate}
% \end{figure}
%
%
In our experiments, we found that 69/188 fixing commits, which cause other issues, are correctly detected by \tool. Meanwhile, the corresponding figures of JITLine and LA\_Predict are 58 and 41, respectively. 
%
Fig.~\ref{fig:RQ1_EX1} shows a commit fixing a bug, yet causing another problem in \textit{FFmpeg}. Specifically, to prevent the out-of-bound problem, \texttt{ch\_data->bs\_num\_env} is set to a valid value if it is larger than the allowance (line 643 in the new version, Fig.~\ref{fig:RQ1_EX1}). However, changing the value of this variable without appropriately checking causes another serious problem, which is later fixed by the commit \texttt{87b08ee}. 
% deleting line 643 in the new version.
%
The dangerous commit in Fig.~\ref{fig:RQ1_EX1} is correctly detected by \tool, while the other methods misclassify this commit as a \textit{safe} one. 


Specifically, the approaches leveraging commit message such as JITLine and JITFine could be misled by special keywords such as ``\textit{Fixes}'' in the commit message:
``\textit{avcodec/aacsbr\_template: Do not leave bs\_num\_env invalid \textbf{Fixes} out of array read \textbf{Fixes}: 1349/clusterfuzz...}''.
%
%
Zeng~\etal~\cite{lapredict} show that the message of a commit could provide the intention of the commit.
However, developers often unintentionally bundle unrelated changes with different purposes (e.g., bug fix and refactoring) in a single commit (tangled commit)~\cite{untangling}.  
% %
Multiple studies have shown that fixing a bug could cause another bug~\cite{guo2010characterizing, purushothaman2005toward}. 
% We also found that various vulnerability-fixing commits actually cause other vulnerabilities.
%
Moreover, in practice, commit messages are often poor-quality, even empty~\cite{good_commit_message}. This makes the application of commit messages for JIT-VD much less reliable and causes incorrect predictions.
%
%
%
Meanwhile, LA\_Predict considers only the line-added-number to evaluate the suspiciousness based on the hypothesis that the larger the line-added-number, the higher the probability of being defective~\cite{lapredict}. In fact, the commit in the example above contains only two added lines of code, which leads to the incorrect prediction of LA\_Predict. 

By capturing the changes in the code structure expressed in the commit's CTG, \tool is able to recognize that the value of \texttt{ch\_data->bs\_num\_env} is dangerously changed (line 643 of the new version) after checking the allowed bound (line 639). In addition, by analyzing the dependencies, \tool can identify that the newly changed value is a magic number (\texttt{2}) and has no relation with the checked bound (\texttt{4}), which means that the corresponding commit still does not guarantee the safety of code after being executed. 
%
Then, this issue is fixed by commit \texttt{87b08ee} (Fig.~\ref{fig:RQ1_EX2}) by using a temporary variable (\texttt{bs\_num\_env}) instead of directly using and defining \texttt{ch\_data->bs\_num\_env}. 
%
As expected, \tool  correctly detects both these two commits.
%
%

% \begin{figure}
%     \centering
%     % \includegraphics[width=0.90\columnwidth]{imgs/ex1-bk.png}
%     \includegraphics[width=0.8\columnwidth]{imgs/ex1.png}
%     \caption{Commit \texttt{a8ad83b} fixing a vulnerability in \textit{FFmpeg} but causing another} 
%     \label{fig:RQ1_EX1}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.9\columnwidth]{imgs/ex2.png}
%     \caption{Commit \texttt{87b08ee} fixing the vulnerability in Fig.~\ref{fig:RQ1_EX1}}
%     \label{fig:RQ1_EX2}
% \end{figure}


\begin{figure}
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
        \centering
    % \includegraphics[width=0.90\columnwidth]{imgs/ex1-bk.png}
        \includegraphics[width=0.7\columnwidth]{imgs/ex1.png}
        \caption{Commit \texttt{a8ad83b} fixing a vulnerability in \textit{FFmpeg} but causing another} 
        \label{fig:RQ1_EX1}
     \end{subfigure}
     \hfill

     \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=0.85\columnwidth]{imgs/ex2.png}
        \caption{Commit \texttt{87b08ee} fixing the vulnerability in Fig.~\ref{fig:RQ1_EX1}}
        \label{fig:RQ1_EX2}
     \end{subfigure}
     
    \caption{Example of a dangerous commit correctly detected by \tool}
\end{figure}
% the pair of safe and dangerous commit



Overall, \textit{properly utilizing the code-related aspects of commits could help} \tool \textit{precisely understand the semantics of the changes and effectively learn to differentiate safe/dangerous commits, thus significantly improves the JIT-VD performance}.




% For example, the dangerous commit in Fig.~\ref{fig:fixing-vt} and the safe (fixing) commit in Fig.~\ref{fig:fixing} are pushed by the same author and have the similar numbers of added lines.
% %
% %
% Meanwhile, \textit{commit messages could be also not reliable for JIT-VD}.
% %
% Zeng~\etal~\cite{lapredict} show that the message of a commit could provide the intent of the commit.
% %
% For example, if a commit's message contains ``\textit{failures}'', ``\textit{fix}'', ``\textit{resolves}'', or ``\textit{task-number}'', then the commit is more likely to be a fixing commit. 
% %
% However, developers often unintentionally bundle unrelated changes with different purposes (e.g., bug fix and refactoring) in a single commit (tangled commit)~\cite{untangling}.  
% %
% Multiple studies have shown that fixing a bugs is likely to result in another bug~\cite{guo2010characterizing, purushothaman2005toward}. We also found that various vulnerability-fixing commits actually cause other vulnerabilities.
% %
% For example, the commit shown in Fig.~\ref{fig:fixing-vt} is dangerous, yet has a message showing its \textit{bug-fixing} intention: \textit{``\textbf{Fixes} use of uninitialized memory''}.
% %
% %
% %
% The commit adds the check for \texttt{avio\_read()} result by removing line 462 in the old version and adding lines 463--464 in the new version to fix the use of uninitialized memory when the call is failed. 
% % %
% However, as show earlier, this unintentionally causes a memory leak. This issue is fixed by commit \texttt{ac480cb} shown in Fig.~\ref{fig:fixing} adding the call of \texttt{av\_free} to free \texttt{extradata} and setting \texttt{extradata\_size = 0} (lines 464--465 of the new version).
% %
% %
% %
% %
% Moreover, in practice, commit messages are often poor-quality, even empty~\cite{good_commit_message}. This makes the application of commit messages for detecting vulnerabilities at the commit level much less reliable.

==> [TSE'23] Just-In-Time Software Vulnerability Detection/7.results/RQ2.tex <==
\subsection{Change Representation Analysis (RQ3)}
\input{7.results/intrinsic/unchanged_parts}

\input{7.results/intrinsic/view_analysis}

\begin{gtheorem}
\textbf{Answer for RQ3}: Besides changed code in CTGs, the related unchanged code significantly contributes to the effectiveness of \tool in detecting dangerous commits. Additionally, incorporating \textit{structure} and \textit{dependency} relations in CTGs enhances the JIT-VD performance of \tool. 
\end{gtheorem}

==> [TSE'23] Just-In-Time Software Vulnerability Detection/7.results/RQ3.tex <==


\subsection{Intrinsic Analysis (RQ2)}
\label{sec:intrinsic}


\input{7.results/intrinsic/attention}

\input{7.results/intrinsic/num_layers}

\input{7.results/intrinsic/aggregation_function}



\begin{gtheorem}
\textbf{Answer for RQ2}: The JIT-VD model's properties/components impact \tool's effectiveness differently. The GNN model and graph readout function slightly impact the performance, while the number of GNN layers could significantly impact \tool's performance.
\end{gtheorem}

==> [TSE'23] Just-In-Time Software Vulnerability Detection/7.results/RQ4.tex <==


\subsection{Sensitivity Analysis (RQ4)}

\subsubsection{Impact of Training Size}

To measure the impact of training data size on \tool's performance, we use the \cross setting, in which the training set is randomly separated into 5 folds.  We gradually  increased the sizes of the training dataset by adding one fold at a time until all the 5 folds are added for training. The results of this experiment are shown in Fig.~\ref{fig:impact_training_size}.
As expected, the performance of \tool is improved when expanding the training dataset. Especially, the precision significantly grows by 38\% when increasing the training size from 1 fold to 5 folds. The reason is that with larger training datasets, \tool has observed more and then performs better. At the same time, training with a larger dataset costs more time. Particularly, the training time of \tool with 5 folds is six times more than the training time with only 1 fold.

\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{imgs/training_size.pdf}
    \caption{Impact of training data size}
    \label{fig:impact_training_size}
\end{figure}





\subsubsection{Impact of Change Complexity}
% In this experiment, we investigate the sensitivity of \tool's inference on the input complexity in number of changed lines. As seen in Fig.~\ref{fig:impact_change_size}, the \textit{precision} of \tool is quite stable with the commits with different complexity levels. 
%
% The the reason could be that using CTGs and the graph-based JIT-VD model make \tool capture precisely 
% the patterns of vulnerabilities at the commit-level. 
%
% However, the number of commits significantly decreases, and there are fewer vulnerability patterns when the complexity is higher.
% However, with larger amounts of changed code, \tool has more information to determine if commits are dangerous or not.
%
% With the smaller sets of dangerous commits and vulnerability patterns, 
% Thus, the proportion of detected ones could be higher, and thus the \textit{recall} is higher.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.9\columnwidth]{imgs/change_size.pdf}
%     \caption{Impact of change size (left axis: precision \& recall; right axis: distribution)}
%     \label{fig:impact_change_size}
% \end{figure}


In this experiment, we investigate the sensitivity of \tool's performance on the input complexity in change rates which are measured by the ratio of the number of changed nodes over the total number of nodes of each CTG (Fig.~\ref{fig:impact_change_size}). As seen, there are much fewer commits (lower distribution - Distr.) with higher complexity levels. Meanwhile, the performance of \tool in both \textit{F1} and \textit{accuracy} is quite stable when handling commits in different change rates. Specifically, the \textit{F1} of \tool gracefully grows from 75\% to 89\%, and the \textit{accuracy} is in the range of 86\% to 89\%, when increasing the change rate.

% if the number of changed nodes is similar to the number of unchanged nodes (changed rate in range 0.5--0.7), \tool'precision is slightly reduced, about 4\%. Meanwhile, the recall is increased when changed rate increases and lightly decreased when all the nodes of the graphs are changed node, i.e., changed rate is 1.0. This is reasonable because 




\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{imgs/change_rate.pdf}
    \caption{Impact of change complexity (left axis: \textit{F1} \& \textit{accuracy}; right axis: Distr.)}
    \label{fig:impact_change_size}
\end{figure}

\begin{gtheorem}
\textbf{Answer for RQ4}: The JIT-VD performance of \tool improves when \tool is trained on a larger  dataset. The performance of \tool in both \textit{F1} and \textit{accuracy} is stable when classifying commits with different change complexity levels.
\end{gtheorem}

==> [TSE'23] Just-In-Time Software Vulnerability Detection/7.results/RQ5.tex <==


\subsection{Time complexity (RQ5)}
In this work, all our experiments were run on a server running Ubuntu 18.04 with an NVIDIA Tesla P100 GPU. 
On average, \tool took less than a second to construct a CTG.
% and produce embeddings for the contents of graph nodes by Word2Vec. 
In \tool, training the JIT-VD model took about 5 hours for 50 epochs. Additionally, \tool with FastRGCN spent 0.75 seconds to classify whether a commit is suspicious or not. 
%


As expected, the more complicated JIT-VD model, the longer the training time. For a fold of data, 1-layer RGAT model took about 40 minutes, while the figures for 3-layer RGAT model and 5-layer RGAT models are 1.5 times and 1.8 times larger. Also, the larger the training dataset, the longer the training time. Specifically, the training time of five folds of data is six times more than that of only one fold. The classification time is not quite different among the variants of \tool. For example, with FastRGCN, the average classification time is 0.75 seconds, while \tool with RGCN took 1.42 seconds to classify a commit.




==> [TSE'23] Just-In-Time Software Vulnerability Detection/7.results/intrinsic/aggregation_function.tex <==
\subsubsection{Impact of Graph Readout Function}

To evaluate the impact of the different readout functions in forming the whole feature vector of a graph, we create different variants of \tool with \textit{Max}, \textit{Average}, and \textit{Sum} function to aggregate node features. 
%
In this experiment, we used the RGAT model, with two layers for the \cross setting.
%
As shown in Table~\ref{tab:impact_readout_function}, \tool's performance is not significantly affected when the aggregation function is changed. Specifically, the average \textit{F1} and \textit{accuracy} are 0.81 and 0.88, respectively.

\begin{table}[]
\centering
\caption{Impact of graph readout function}
\label{tab:impact_readout_function}
\begin{tabular}{@{}l|rrr|r@{}}
\toprule
                    & \textit{Precision} & \textit{Recall}   & \textit{F1}   & \textit{Accuracy}  \\ \midrule
\textit{Max}  & 0.93	            & 0.73	            & 0.81	        & 0.88           \\
\textit{Average}     & 0.92               & 0.73          & 0.81            & 0.88           \\
\textit{Sum}     & 0.95               & 0.70          & 0.80          & 0.87       \\

\bottomrule
\end{tabular}
\end{table}

==> [TSE'23] Just-In-Time Software Vulnerability Detection/7.results/intrinsic/attention.tex <==
\subsubsection{Impact of GNN Model}
To investigate the impact of different GNN models on the JIT-VD performance, we compare three variants of relational graph networks: \tool with RGCN~\cite{rgcn},  RGAT~\cite{rgat},  and  FastRGCN~\cite{fastgcn}. 
%
In this experiment, we used the \textit{sum} readout function and two GNN layers, and applied for the \dev setting.
%
The results of those three variants is shown in Table~\ref{tab:gnn_models}. As expected, \tool obtains quite stable performance with about 0.74\% in \textit{F1} and 0.85 in \textit{accuracy}.
Moreover, while \tool obtains quite similar \textit{precision} and \textit{recall} with both RCGN and FastRGCN, it archives the highest \textit{precision}, yet lowest \textit{recall} with RGAT.
Indeed, the attention mechanism enables RGAT to focus on the important features of the neighboring nodes in each relation for computing the features of the graph nodes. This helps RGAT precisely detect dangerous commits and obtains the highest \textit{precision}. However, 
% it could also cause the models to suffer from over-fitting problem affecting the \textit{recall} performance.
the attention mechanism in the RGAT model may be causing it to prioritize certain features, leading to higher \textit{precision} but lower \textit{recall}. This can happen if the attention mechanism is too focused on specific features and fails to capture the broader context of the data.

\begin{table}[]
\centering
\caption{Impact of GNN models on JIT-VD Performance}
\label{tab:gnn_models}
\begin{tabular}{@{}l|rrr|r@{}}
\toprule
                    & \textit{Precision} & \textit{Recall}   & \textit{F1}   & \textit{Accuracy}  \\ \midrule
RGCN  & 0.78	            & 0.70	            & 0.74	        & 0.85           \\
FastRGCN     & 0.77               & 0.71          & 0.74            & 0.85       \\
RGAT     & 0.82               & 0.66          & 0.73            & 0.85           \\
% CuGraphRGCNConv     & 0.82               & 0.66          & 0.73            & 0.85  \\
\bottomrule
\end{tabular}
\end{table}

==> [TSE'23] Just-In-Time Software Vulnerability Detection/7.results/intrinsic/feature_engineering.tex <==
\subsubsection{Impact of Feature Engineering}
\begin{table}[]
\centering
\caption{Impact of Feature Engineering}
\label{tab:feature_engineering}
\begin{tabular}{@{}lrrrrr@{}}
\toprule
                        & \textit{Precision} & \textit{Recall}   & \textit{F1}   & \textit{Accuracy} \\ \midrule
Word2vec                 & XXX               & XXX          & XXX                 & XXX               \\
FastText                & XXX               & XXX          & XXX                & XXX                \\
CodeBERT         & XXX	             & XXX         & XXX	             & XXX	             \\
\bottomrule
\end{tabular}
\end{table}

==> [TSE'23] Just-In-Time Software Vulnerability Detection/7.results/intrinsic/num_layers.tex <==
\subsubsection{Impact of Number of GNN Layers}

To study the impact of the number of GNN layers on the JIT-VD performance of \tool, we varied the number of GNN layers in JIT-VD model from 1 to 5. 
%
In this experiment, we used RGAT for the JIT-VD model and the \dev setting.
%
As seen in Fig.~\ref{fig:impact_num_layers}, the JIT-VD \textit{F1} and classification \textit{accuracy} of \tool are significantly better when increasing the number of RGCN layers in the JIT-VD model from one to two. With two RGCN layers, the model represents each node in CTGs from the 2-hop neighborhood. Meanwhile, each node is represented by considering only its neighbors by the model with one RGCN layer.
Thus, by using more information to represent each node in CTGs, the model detected dangerous commits more precisely. Indeed, the precision of \tool is  remarkably improved by 67\% with two RGCN layers. As expected, the more complex node representation mechanism slightly lowers the recall by 7\%.
%
However, considering longer 2-hop neighborhood to represent nodes in CTGs causes downgrades in the detection performance. Particularly, the performance \tool gracefully decreases when the number of GNN layers increases from 2 to 5. This could be because for a node, the further information collected from the other nodes could bring noises in representing the node. Additionally, with a larger number of layers and a longer neighborhood relation, the set of the shared neighbors which are used to represent nodes could be larger. Thus, the different nodes could be represented similarly. Consequently, the discriminating performance of GNN model is reduced.
%
Moreover, the model with more layers is much more complicated. Thus, we use two GNN layers to ensure the best performance and simplicity.






\begin{figure}[!h]
    \centering
    \includegraphics[width=0.9\columnwidth]{imgs/num_layers.pdf}
    \caption{Impact of the number of GNN layers}
    \label{fig:impact_num_layers}
\end{figure}


==> [TSE'23] Just-In-Time Software Vulnerability Detection/7.results/intrinsic/predic_model.tex <==
\begin{table}[]
\centering
\caption{Impact of Prediction Model}
\label{tab:predict_model}
\begin{tabular}{@{}lrrrrr@{}}
\toprule
                        & \textit{Precision} & \textit{Recall}   & \textit{F1}   & \textit{Accuracy} \\ \midrule
MLP                & XXX               & XXX          & XXX                 & XXX               \\
Logistic Regression                 & XXX               & XXX          & XXX                & XXX                \\
Gradient Boosting Machine          & 0.82	             & 0.66	         & 0.73	             & 0.85	             \\
Random Forest   & 0.86	             & 0.62	         & 0.72	             & 0.85	             \\
\bottomrule
\end{tabular}
\end{table}

==> [TSE'23] Just-In-Time Software Vulnerability Detection/7.results/intrinsic/unchanged_parts.tex <==
%
\subsubsection{Unchanged Code's Role Analysis}
To investigate the contribution of the related unchanged code in CTGs, we used two variants of CTG: one considering both changed code and unchanged code (CTG), the other considering only changed code ($\hat{\text{CTG}}$). Table~\ref{tab:unchanged-code} shows the JIT-VD performance of \tool using the two CTG variants: $\tool_\text{CTG}$ and $\tool_{\hat{\text{CTG}}}$. 
%
Note that, in this experiment, we applied for the \cross setting and used the same RGAT model, with two layers, and sum readout function for both CTG variants.

As seen, additionally considering the related unchanged code along with changed code in CTGs significantly improves the JIT-VD performance of \tool using CTGs with only changed code. Particularly, \tool achieves better \textit{precision} and \textit{recall} by 20\% and 15\%, respectively. 
The related unchanged code provides valuable information and helps the model not only understand code changes more precisely but also discover more vulnerability patterns. 
%
The number of dangerous commits detected by $\tool_\text{CTG}$ but not detected by $\tool_{\hat{\text{CTG}}}$ (149 commits) nearly triples the corresponding figure by $\tool_{\hat{\text{CTG}}}$ but not detected by $\tool_\text{CTG}$ (only 52 commits).
%
This experimentally confirms our observation 2 on the important role of related unchanged code for understanding code changes in JIT-VD.



\begin{table}[]
\centering
\caption{Impact of the unchanged code in CTGs on \tool's performance}
\label{tab:unchanged-code}
\begin{tabular}{l|rrr|r}
\toprule
                       & \textit{Precision} & \textit{Recall} & \textit{F1} & \textit{Accuracy} \\ \midrule
$\tool_\text{CTG}$    & 0.95               & 0.70            & 0.80        & 0.87              \\
$\tool_{\hat{\text{CTG}}}$ & 0.79               & 0.61            & 0.69        & 0.79              \\ \bottomrule
\end{tabular}
\end{table}

==> [TSE'23] Just-In-Time Software Vulnerability Detection/7.results/intrinsic/view_analysis.tex <==
\subsubsection{Code Relation Analysis}
To analyze the impact of the relations in CTGs, we used different variants of CTGs: $\mathcal{R} = \{\textit{structure}\}$, $\mathcal{R} = \{\textit{dependency}\}$, and $\mathcal{R} = \{\textit{structure, dependency}\}$. In this experiment, we used the same setting for JIT-VD model (RGAT model having two layers, and \textit{sum} readout function) for all the variants, and applied in the \dev setting.

As seen in Table~\ref{tab:view_analysis}, \tool performs quite stably when $\mathcal{R} = \{\textit{structure}\}$ and $\mathcal{R} = \{\textit{dependency}\}$, i.e., \textit{F1 = 0.69} in both cases. When combining both relations in CTGs, \tool detects the dangerous commits significantly more precisely while its \textit{recall} remains stable. It is reasonable because considering both the structure relation and the dependency relation in CTGs gains the information that is necessary for the model to determine if a commit is suspiciously dangerous. As a result, both the JIT-VD \textit{F1} and \textit{accuracy} increase when $\mathcal{R} = \{\textit{structure, dependency}\}$. 
%

Since several existing studies consider the execution flow (i.e., control flow) relation between program elements in detecting vulnerabilities~\cite{gascon2013structural, sparks2007automated}, we additionally consider $\mathcal{R} = \{\textit{structure, dependency, exec. flow}\}$ in CTGs to evaluate the expandability of our proposed code change representation. We found that additionally considering the execution relation in CTGs, $\mathcal{R} = \{\textit{structure, dependency, exec. flow}\}$, decreases the performance of \tool by 1.4\% in \textit{F1}. As expected, in this case, the \textit{precision} is 4.8\% better than that of \tool with $\mathcal{R} = \{\textit{structure, dependency}\}$. Nevertheless, the changes in the execution flow (i.e., control flow), that are required for determining dangerous commits, could be covered by the changes in the dependency relation via control dependencies. This redundancy hurts \tool's recall 6.1\%. Moreover, this conditional consideration increases the complexity of CTGs and the cost for training and testing the JIT-VD model.
%
Thus, in this work, we use $\mathcal{R} = \{\textit{structure, dependency}\}$ in CTGs for the best performance and efficiency of \tool.


\begin{table}[]
\centering
\caption{Impact of the code relations on \tool's performance}
\label{tab:view_analysis}
\begin{tabular}{@{}l|rrr|r@{}}
\toprule
                        & \textit{Precision} & \textit{Recall}   & \textit{F1}   & \textit{Accuracy} \\ \midrule
Struct.                 & 0.72	             & 0.66	             & 0.69	         & 0.82               \\
Depend.                 & 0.70	             & 0.69	             & 0.69	         & 0.81               \\
Struct.+Depend.         & 0.82	             & 0.66	             & 0.73	         & 0.85	             \\
% Struct.+Depend.+Control.   & 0.86	             & 0.62	             & 0.72	         & 0.85	             \\
\bottomrule
\end{tabular}
\end{table}
















% To analyze the impact of the relations in CTGs, we used different variant of CTGs: $\mathcal{R} = \{\textit{structure}\}$, $\mathcal{R} = \{\textit{dependency}\}$, $\mathcal{R} = \{\textit{structure, dependency}\}$, and $\mathcal{R} = \{\textit{structure, dependency, control-flow}\}$. In this experiment, we used the same setting for JIT-VD model (RGAT model having two layers, and \textit{sum} readout function) for all the variants, and applied for the \dev setting.

% As seen in Table~\ref{tab:view_analysis}, \tool performs quite stably when $\mathcal{R} = \{\textit{structure}\}$ and $\mathcal{R} = \{\textit{dependency}\}$, i.e., \textit{F1 = 0.69} in both cases. When combining both the two relations in CTGs, \tool detects the dangerous commits significantly more precisely while its \textit{recall} is remained stable. It is reasonable because considering both the structure relation and the dependency relation in CTGs gains the information that is necessary for the model to determine if a commit is suspiciously dangerous. As a result, both the JIT-VD \textit{F1} and \textit{accuracy} increase when $\mathcal{R} = \{\textit{structure, dependency}\}$. 
% %

% Additionally considering the execution relation (i.e., control flow) in CTGs, $\mathcal{R} = \{\textit{structure, dependency, control-flow}\}$, decreases the performance of \tool by 1.4\% relatively. As expected, in this case, the precision is 4.8\% better when $\mathcal{R} = \{\textit{structure, dependency}\}$. Nevertheless, the changes in control flow (execution flow), that are required for determining dangerous commits, could be covered by the changes in the dependency relation via control dependencies. This redundancy hurts \tool's recall 6.1\%. Moreover, this conditional consideration increases the complexity of CTGs and the cost for training and testing the JIT-VD model.
% %
% Thus, in this work, we use $\mathcal{R} = \{\textit{structure, dependency}\}$ in CTGs for the best performance and efficiency.


% \begin{table}[]
% \centering
% \caption{Impact of Relation on Performance}
% \label{tab:view_analysis}
% \begin{tabular}{@{}lrrrrr@{}}
% \toprule
%                         & \textit{Precision} & \textit{Recall}   & \textit{F1}   & \textit{Accuracy} \\ \midrule
% Struct.                 & 0.72	             & 0.66	             & 0.69	         & 0.82               \\
% Depend.                 & 0.70	             & 0.69	             & 0.69	         & 0.81               \\
% Struct.+Depend.         & 0.82	             & 0.66	             & 0.73	         & 0.85	             \\
% Struct.+Depend.+Control.   & 0.86	             & 0.62	             & 0.72	         & 0.85	             \\
% \bottomrule
% \end{tabular}
% \end{table}

==> [TSE'23] Just-In-Time Software Vulnerability Detection/7.results/threats.tex <==
\subsection{Threats to Validity}
The main threats to the validity of our work consist of internal, construct, and external threats.

\textbf{Threats to internal validity} include the influence of the method used to construct relational code graph and identify the relation between program entities. To reduce this threat, we use Joern~\cite{joern} code analyzer, which is widely used in existing studies~\cite{velvet,vuldeeppeaker,ivdetect,linevd}. Another threat mainly lies in the correctness of the implementation of our approach. To reduce such threat, we carefully reviewed our code and made it public~\cite{CodeJIT} so that other researchers can double-check and reproduce our experiments.



\textbf{Threats to construct validity} relate to the suitability of our evaluation procedure. We used \textit{precision}, \textit{recall}, \textit{F1}, and classification \textit{accuracy}. They are the widely-used evaluation measures for \jit defect detection~\cite{jit-fine,jitline,lapredict} and \jit vulnerability detection~\cite{vccfinder,vuldigger}. 
%
Besides, a threat may come from the adaptation of the baseline approaches. To mitigate this threat, we directly obtain the original source code from the GitHub repositories of the studied techniques. Also, we use the same hyperparameters as in the original papers~\cite{jit-fine,jitline,lapredict,vccfinder,deepjit}. 

\textbf{Threats to external validity} mainly lie in the selection of graph neural network models used in our experiments. 
To mitigate this threat, we select the representative models which are well-known for NLP and SE tasks~\cite{rgcn,rgat,fastgcn}. 
In addition, the construction of our dataset is another threat which is also suffered by related studies~\cite{lapredict, vccfinder, are_we_there}. 
%
Specifically, the commits triggering/contributing to vulnerabilities are considered as dangerous ones.
%
% To reduce the impact of this threat, we consider program dependencies during collecting dangerous commits and focus on the vulnerability triggering commits as the dangerous commits instead of vulnerability contributing commits 
%
To reduce the impact of this threat, we focus on the vulnerability triggering commits as the dangerous commits instead of vulnerability contributing commits. Also, to precisely blame vulnerable statements during collecting dangerous commits, we consider program dependencies instead of surrounding statements as mentioned in Sec.~\ref{sec:data}. 
%
%
Another threat is considering the vulnerability-fixing commits as safe ones because these commits could contribute to vulnerabilities. To reduce this threat, only the fixing commits which are not VCCs are considered as safe.
%
Moreover, our experiments are conducted on only the code changes of C/C++ projects. Thus, the results could not be generalized for other programming languages. In our future work, we plan to conduct more experiments to validate our results to other languages. 

% \tool is considered as the baseline approach for general multi-label text classification, while all Word2vec, Glove, and CodeBERT are reputed and shown to be effective in many SE tasks. 
% %
% The dataset used in our experiments might not be representative or not very high-quality. To reduce this threat, we used the largest public dataset~\cite{bigvul}, which is collected from a large number of real-world projects and widely used in existing vulnerability detection studies~\cite{linevd, linevul, ivdetect}. Additionally, our data has only C/C++ code. Thus, we cannot claim that similar results would have been observed in other programming languages. Further studies are needed to validate and generalize our findings to other languages.

%Limitation: Bugs related to lexical --> change order of parameters


==> [TSE'23] Just-In-Time Software Vulnerability Detection/8.related-work.tex <==
\section{Related Work}
\tool relates to the work on \textbf{just-in-time vulnerability detection}~\cite{vccfinder, vuldigger}. 
VCCFinder~\cite{vccfinder} and VulDigger~\cite{vuldigger} are the classification models combining code-metrics, commit messages, and expert features for JIT-VD.
Meanwhile, the work on \textbf{just-in-time bug detection}~\cite{jit-fine,jitline,lapredict,deepjit} could also be applied to detect vulnerabilities at the commit-level. DeepJIT~\cite{deepjit} automatically extracts features from commit messages and changed code and uses them to identify defects. Pornprasit~\etal propose JITLine, a simple but effective just-in-time defect prediction approach. JITLine utilizes the expert features and token features using bag-of-words from commit messages and changed code to build a defect prediction model with random forest classifier. 
LAPredict~\cite{lapredict} is a defect prediction model by leveraging the information of "lines of code added" expert feature with the traditional logistic regression classifier. 
Recently, Ni~\etal introduced JITFine~\cite{jit-fine} combining the expert features and the semantic features which are extracted by CodeBERT~\cite{codebert} from changed code and commit messages. 
%
%
%
Different from all prior studies in \jit bug/vulnerability detection, our work presents the first study centralizing the role of code change semantics in detecting vulnerabilities at the commit level. In \tool, the code change meaning is the only deciding factor in examining the suspiciousness of commits. Our results experimentally show that our strategy is more appropriate for JIT-VD.

% \tool also relates to the studies on \textbf{just-in-time bug localization}~\cite{localization2phase,deep_localization}.

\textbf{Vulnerability detection} is also a critical part to be discussed. Various methods have been proposed to determine if a code component (component, file, function/method, or statement/line) is vulnerable. 
% The rule-based techniques apply static analyzers and leverage seen vulnerability patterns, such as FlawFinder~\cite{FlawFinder} or Coverity~\cite{Coverity}. 
Recently, several deep-learning based approaches have been introduced~\cite{survey_papers, poster, vuldeeppeaker, vulsniper, devign, are_we_there,mvd,issta_22}. 
VulDeePecker~\cite{vuldeeppeaker} and SySeVR~\cite{sysevr} introduce tools to detect \textit{slice-level} vulnerabilities, which are more fine-grained.
IVDetect~\cite{ivdetect}, which is a graph-based neural network model, is proposed to detect vulnerabilities at the function level and use a model interpreter to identify vulnerable statements in the detected suspicious functions. LineVul~\cite{linevul} and LineVD~\cite{linevd} apply CodeBERT in their own way and have been shown that they are more effective than IVDetect in detecting vulnerable functions and lines/statements. VelVet~\cite{velvet} builds graph-based models to detect vulnerable statements.
%
%
Those approaches focus on detecting vulnerabilities at the release-time, while \tool is a \jit vulnerability detection. \tool and the release-time approaches could complement to support developer in ensuring software quality in the development process.  

% \textbf{Change representation}. CPathMiner~\cite{cpathminer}

% \textbf{Change representation learning}. cc2vec~\cite{cc2vec}, CodeReviewer~\cite{codereviewer},

Several \textbf{learning-based approaches} have been proposed for specific SE tasks including code suggestion~\cite{icse20, naturalness, allamanis2016convolutional}, program synthesis~\cite{amodio2017neural,gvero2015synthesizing}, pull request description generation~\cite{hu2018deep,liu2019automatic}, code summarization~\cite{iyer2016summarizing,mastropaolo2021studying,wan2018improving}, code clones~\cite{li2017cclearner}, fuzz testing\cite{godefroid2017learn}, bug detection~\cite{oppsla19}, and program repair~\cite{jiang2021cure,ding2020patching}.


==> [TSE'23] Just-In-Time Software Vulnerability Detection/9.conclusion.tex <==
\section{Conclusion}
%
In this paper, we propose \tool, a novel code-centric approach for just-in-time vulnerability detection (JIT-VD). 
%
Our key idea is that \textit{the meaning of the changes in source code caused by a commit is the direct and deciding factor for assessing the commit's riskiness.}
%
We design a novel graph-based multi-view code change representation of the changed code of commits in relation to the unchanged code. Particularly, a graph-based JIT-VD model is developed to capture the patterns of dangerous/safe (benign) commits and detect vulnerabilities at the commit level. 
%
%
%
%
On a large public dataset of dangerous and safe commits, our results show that \tool significantly improves the state-of-the-art JIT-VD methods by up to 66\% in \textit{Recall}, 136\% in \textit{Precision}, and 68\% in \textit{F1}. 
%
Moreover, \tool correctly classifies nearly 9/10 of dangerous/safe  commits. 
%


==> [TSE'23] Just-In-Time Software Vulnerability Detection/problem.tex <==
Software is an important element of the infrastructure of the modern economy and society. Software vulnerability attacks target computer software systems, especially important systems such as national citizen data management, traffic, aviation coordination, and transportation. chemical/nuclear industrial operations, and national security systems, can cause significant damage. According to Veracode's survey of more than 130,000 software in 2020, more than 75\% of which contain at least one software vulnerability. Common vulnerabilities include: broken access control, cryptographic failures, SQL injections, insecure design, and wrong security configuration. According to a survey by Synopsys in 2021 with a total of 2,409 software, 97\% of the software in those software contains open source. 80\% of them contain at least one open source vulnerability. Notably, at the end of 2021, a new (zero-day) vulnerability in the popular Apache engine, Log4j was discovered. The vulnerability, known as Log4Shell (CVE-2021-44228), allows hackers to arbitrarily execute code on vulnerable servers. Many commercial cloud services are affected by this vulnerability including Amazon Web Services, Cloudflare, iCloud, Minecraft: Java version, Steam, Tencent QQ and many more. According to estimates [4], Log4Shell impacted 93\% of enterprise cloud environments. In fact, according to the latest survey of the Society for Software & Information Quality (CISQ) released in 2021, the total cost of bugs related to software vulnerabilities in the US (accounting for 33\% of the market share in the US). world technology market) by 2020 to 1.56 trillion USD. This cost accounts for 75\% of the cost caused by poor quality software.
In Vietnam, in 2021, the Ministry of Public Security recorded 8 million attack warnings with 2,763 attacks targeting the domestic electronic information system (up 26\% compared to 2020), many of which were software systems of state agencies [25]. According to statistics, more than 75\% of attacks on critical systems recorded in 2021 are exploiting hardware and software vulnerabilities [26]. Attacks to exploit such vulnerabilities can lead to damage in many ways to individuals, groups, and even affect national security. Therefore, as a part of network security, software security is increasingly concerned and determined by the Party and State in the country's development orientation, especially in the period when the country accelerates digital transformation.
To minimize the consequences caused by vulnerabilities in software, as recommended by CISQ, software vulnerabilities should be detected and fixed/prevented as soon as possible, because of late detection and correction. can cost 200 times more, or even cause more serious damage. To detect and prevent software vulnerabilities early, solutions being applied in the software industry include following safe design principles, manually reviewing security best practices. software (security best practices), and software testing. The most effective solution being applied in practice is to use techniques that automatically detect software vulnerabilities in the source code before deployment. Current automated software vulnerability detection techniques fall into two main categories: static code analysis techniques and data-driven techniques.
Static code analysis techniques including similarity-based and pattern-based such as Sonaque, Klocwork, Coverity, or Polyspace are widely used in industry. Similarity-based tools can identify vulnerabilities caused by code clones/reuses, but often produce a large number of warnings with a high false positive rate. positive). Methods using patterns require experts to define rules/features that represent vulnerabilities. This requirement makes sample methods prone to error and laborious. Therefore, an ideal method should be able to efficiently detect vulnerabilities caused by multiple causes while imposing as little reliance on human experts as possible.
Data-driven vulnerability detection using pattern regconition and machine learning provides alternative solutions for more efficient and automated vulnerability detection [15-17]. Machine learning algorithms can learn abstract patterns of potentially vulnerable source code. The researchers applied source code features such as imports, function calls, and software complexity metrics as metrics to identify likely files or pieces of code being attacked.
The emerging use of deep learning techniques provides new potential for the field of vulnerability detection using machine learning. On the one hand, the hierarchical structure of deep learning models helps to facilitate the learning of highly abstract and non-linear patterns that are capable of capturing

==> [TSE'23] Just-In-Time Software Vulnerability Detection/tables/tab-inspection-comparison.tex <==
\begin{table}[]
\centering
\caption{\textit{Development-process}: JIT-VL Performance Comparison}
\label{tab:vl-perf-time}
\begin{tabular}{@{}llllll@{}}
\toprule
         & top-1 & top-3 & top-5 & top-10 & MRR \\ \midrule
SN-based &       &       &       &        &     \\
JITLine &       &       &       &        &     \\
JITFine  &       &       &       &        &     \\
\tool    &       &       &       &        &     \\ \bottomrule
\end{tabular}
\end{table}

\begin{table}[]
\centering
\caption{\textit{Cross-project}: JIT-VL Comparison}
\label{tab:vl-perf-proj}
\begin{tabular}{@{}llllll@{}}
\toprule
         & top-1 & top-3 & top-5 & top-10 & MRR \\ \midrule
SN-based &       &       &       &        &     \\
JITLine &       &       &       &        &     \\
JITFine  &       &       &       &        &     \\
\tool    &       &       &       &        &     \\ \bottomrule
\end{tabular}
\end{table}

==> [TSE'23] Just-In-Time Software Vulnerability Detection/tables/tab-jit-vd-comparison.tex <==
% \begin{table}[]
% \centering
% \caption{\textit{Development-process: }JIT-VD Performance Comparison}
% \label{tab:vd-perf-time}
% \begin{tabular}{@{}llllll@{}}
% \toprule
%                    & \textit{Precision} & \textit{Recall} & \textit{F1}   & \textit{Accuracy} & \textit{AUC}  \\ \midrule
% VCCFinder          &                    &               &      &          &      \\
% CC2Vec+DeepJIT     & 0.33               & 0.66          & 0.44            & 0.49            & 0.52 \\
% LA\_Predict        & 0.59               & 0.58          & 0.59            & 0.75            & 0.77 \\
% JITLine            & 0.68	            & 0.56	        & 0.62	          & 0.79	        & 0.80 \\
% JITFine            & 0.62	            & \textbf{0.73}	& 0.67	          & 0.78	        & \textbf{0.83} \\
% \tool              & \textbf{0.82}	    & 0.66	        & \textbf{0.73}	  & \textbf{0.85}	& 0.82 \\ \bottomrule
% \end{tabular}
% \end{table}


% \begin{table}[]
% \centering
% \caption{\textit{Cross-project}: JIT-VD Performance Comparison}
% \label{tab:vd-perf-proj}
% \begin{tabular}{@{}llllll@{}}
% \toprule
%                    & \textit{Precision}  & \textit{Recall}    & \textit{F1}    & \textit{Accuracy}  & \textit{AUC}  \\ \midrule
% VCCFinder          &            &           &       &           &      \\
% CC2Vec+DeepJIT     & 0.40	    & 0.69	    & 0.51	& 0.50	    & 0.52  \\
% LA\_Predict        & 0.66	    & 0.48	    & 0.56	& 0.72	    & 0.75  \\
% JITLine            & 0.62	    & 0.63	    & 0.62	& 0.72	    & 0.76 \\
% JITFine            & 0.68	    & 0.69	    & 0.68	& 0.76	    & 0.82     \\
% \tool              & \textbf{0.95}	    & \textbf{0.70}	    & \textbf{0.80}	& \textbf{0.87}	    & \textbf{0.88} \\ \bottomrule
% \end{tabular}
% \end{table}







\begin{table}[]
\centering
\caption{\textit{Dev.-process:} JIT-VD performance comparison}
\label{tab:vd-perf-time}
\begin{tabular}{@{}l|rrr|r@{}}
\toprule
                   & \textit{Precision} & \textit{Recall} & \textit{F1}   & \textit{Accuracy} 
                   % & \textit{AUC}  
                   \\ \midrule
VCCFinder          & 0.50	            & \textbf{0.75}	        & 0.60	          & 0.70           \\
CC2Vec+DeepJIT     & 0.33               & 0.66          & 0.44            & 0.49            \\
LA\_Predict        & 0.59               & 0.58          & 0.59            & 0.75            \\
JITLine            & 0.62	            & 0.66	        & 0.64	          & 0.77	        \\
JITFine            & 0.62	            & 0.73	        & 0.67	          & 0.78	        \\
\tool              & \textbf{0.78}	    & 0.70	        & \textbf{0.74}	  & \textbf{0.85}	\\ \bottomrule
\end{tabular}
\end{table}


\begin{table}[]
\centering
\caption{\textit{Cross-project}: JIT-VD performance comparison}
\label{tab:vd-perf-proj}
\begin{tabular}{@{}l|rrr|r@{}}
\toprule
                   & \textit{Precision}  & \textit{Recall}    & \textit{F1}    & \textit{Accuracy}  \\ \midrule
VCCFinder          & 0.58	    & 0.49	    & 0.53	& 0.74          \\
CC2Vec+DeepJIT     & 0.40	    & 0.69	    & 0.51	& 0.50	    \\
LA\_Predict        & 0.66	    & 0.48	    & 0.56	& 0.72	    \\
JITLine            & 0.57	    & 0.72	    & 0.64	& 0.69	    \\
JITFine            & 0.68	    & 0.69	    & 0.68	& 0.76	    \\
\tool              & \textbf{0.90}	& \textbf{0.80}	& \textbf{0.84}	& \textbf{0.89} \\ \bottomrule
\end{tabular}
\end{table}

==> [TSE'23] Just-In-Time Software Vulnerability Detection/tasks/task1.tex <==





\subsection{Task 1: Construction of a large dataset of dangerous \& safe commits and an empirical study}
\label{sec:task_1}
This section discusses our design, preliminary results, and a plan for a user study to collect and validate a large dataset of dangerous commits of software systems' repositories.
%
To facilitate applying advanced machine learning techniques automatically and effectively learning latent and abstract dangerous commit patterns, our goal is to collect a large number of dangerous and safe commits in numerous real-world projects. Therefore, we plan to perform a semi-automated data collection process (Figure~\ref{fig:process}). 

Particularly, from various vulnerability datasets~\cite{fixing_database1,bigvul}, \textbf{(1)} we are extracting the vulnerability-fixing commits which can be considered as \textit{safe commits}~\cite{vccfinder,are_we_there,vuldigger}. 
%
To identify \textit{dangerous commits}/\textit{vulnerability contributing commits (VCCs)}, the general idea is to start from vulnerable statements and identify the commits which modify these statements. \textbf{(3)} This can be done by using \texttt{git blame}. 
%
\textbf{(2)} The vulnerable statements are identified thanks to the fixing commits based on the following heuristics. 
%
The statements which are deleted by the fixing commits could be considered to be vulnerable~\cite{vccfinder,vuldigger, vul_secret, bigvul}. 
%
For the statements added by the fixing commits, the existing studies~\cite{vccfinder,vuldigger} assume that the \textit{physically} surrounding statements are vulnerable, regardless of whether these statements semantically relate to added statements or not. This procedure could miss the actually vulnerable commits and incorrectly blame safe commits. To reduce this risk, we are starting from the statements which are \textit{semantically} related to the added statements rather than the surrounding ones.
%
Since the method of identifying vulnerable statements is based on heuristics, it could cause inaccuracy in collecting VCCs. \textbf{(4)} We plan to sample the collected commits and manually read vulnerability reports as well as source files to validate the identified VCCs, then refine our heuristics if necessary.


\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{imgs/dataset.png}
    \caption{A Semi-automated Data Collection Process}
    \label{fig:process}
\end{figure}

% \subsubsection{}
\textbf{Summarized preliminary results}. In this ongoing task, we have done Step 1 -- Step 3. In total, we have collected 14K fixing commits from the vulnerabilities reported from Jan 1990 - Aug 2022 in real-world 603 C/C++ projects such as Ffmpeg, Qemu, Linux, Chromium, and Tensorflow. There are 44K VCCs corresponding to the fixing commits. We are working on validating the heuristics used in identifying VCCs and refining our heuristics to improve the data collection procedure (Step 4). This process provides us with several observations: 


1. We found many cases violating the principle on commit matrices (e.g., developers' experience or numbers of added/deleted lines) used to detect risky commits in the existing studies~\cite{vuldigger,vccfinder}. 

2. Meanwhile, deciding if a change is dangerous/safe requires understanding certain code characteristics of not only the change but also its relevance to the unchanged parts and how the change affects code structure, execution, and dependencies. 

\textbf{Future activities}. We plan to investigate VCCs further to gain more knowledge about them. We will investigate the resolution process of VCCs by studying the corresponding fixing commits to know how they are resolved. We will examine more repositories on software vulnerabilities. Our goal is to answer the following research questions:

- R1: How complex are the vulnerabilities caused by dangerous commits (in terms of involving code statements, functions, or files)?

- R2: Which characteristics of code contribute to the riskiness/safeness of commits? 

- R3: Whether different dangerous/safe commits in different code components/projects share some similar characteristics?

==> [TSE'23] Just-In-Time Software Vulnerability Detection/tasks/task2.tex <==
\subsection{Task 2: Scientific Foundation for Representations, Dangerous Commit Detection, and Fine-Grained Interpretations}
\label{sec:task_1}

The goal of this task is to investigate the scientific foundation, including the concepts, representations, models, techniques, and tools to detect vulnerabilities at the commit level. Let us describe our ideas on the concepts and models to represent code changes, detect dangerous commits, and provide explanations for predictions as hints for the further interpretation of developers.

% \begin{figure}
%     \centering
%     \lstinputlisting[language=C]{examples/example.c}
%         \caption{CVE-2016-6156}
%         \label{fig:BO_vul_ex}
% \end{figure}

\subsubsection{Semantic Fine-Grained Code Transformation Representation}
\label{sec:ctg}
% In our prior work~\cite{cpathminer}, we had developed a graph-based model to represent code changes. In general, this model represents a code change by two graph method calls, variable declarations, operations, or control statements as nodes and control/data dependencies as edges. Using GROUMs, we have successfully mined object usage patterns in the programs. Usage patterns could be considered as class/method reuse and/or API reuse. Therefore, based on that model, we propose to represent vulnerability models by graphs. Each vulnerability model is a graph in which:


% 
The goal of this sub-task is to define important concepts and models to represent changes. Our key research question is R4: How to represent a code change to support understanding the change and determining its safeness/riskiness for the source code?

Based on our code-centric philosophy in just-in-time vulnerability detection and our observations from the ongoing Task 1, we plan to represent changes by the models which can capture the code semantics and the code transformation caused by the changes. The changes will be represented in the context of the unchanged parts, as well as the code transformations in the syntactic structure, execution flow, and dependencies. Once the code-centric models of the changes are built, we could employ a machine-learning model and interpreting methods to learn detecting dangerous changes and provide code-related explanations for the model's predictions.


From our point of view, a program is a set of \textit{inter-related elements} and \textit{relations} and \textit{dependencies} with other entities. The relations and dependencies of the code elements could be captured in graphs~\cite{cpathminer}. 
%
%
%
Thus, we plan to propose a graph-based representation that connects elements involved in changes when they have \textit{structural} relation, \textit{control-flowing} relation, or \textit{dependencies}. 
%
%
%
Particularly, each commit is represented as a \textit{Code Transformation Graph (CTG)} which is an annotated graph, $G = \langle N, E, \alpha \rangle$:
\begin{itemize}[noitemsep]
    \item Nodes in $N$ represent the code elements in the changed and unchanged parts.
    \item Edges in $E$ represent either the structural, control-flowing, or data/control dependency relations between nodes.
    \item Annotations for nodes and edges are either \textit{remained}, \textit{added}, or \textit{deleted} by the change. Formally, $\alpha(g) \in \{$\textit{remained}, \textit{added}, \textit{deleted}$\}$, where $g$ is a node in $N$ or an edge in $E$.
\end{itemize}
%
Our idea to construct the CTG, $G = \langle N, E, \alpha \rangle$, of a commit is combining the \textit{code property graphs (CPGs)}~\cite{cpg} of the old version ($G_o = \langle N_o, E_o \rangle$) and the new one ($G_n = \langle N_n, E_n \rangle$). By merging its \textit{abstract syntax tree (AST)}, \textit{control-flow graph (CPG)}, and \textit{program dependence graph (PDG)}, these graphs capture the syntactic structure, execution flow, and dependencies of the code \textit{version} before and the one after the commit. Specially, $G = \langle N, E, \alpha \rangle$ is constructed from $G_o = \langle N_o, E_o \rangle$ and $G_n = \langle N_n, E_n \rangle$ as follows: $N = N_o \cup N_n$, $E = E_o \cup E_n$, and for a graph element $g$ (i.e., a node or an edge of $G$):
%
\begin{itemize}[noitemsep]
    \item $\alpha(g) =$ \textit{added} if $g$ is a node and $g \in N_n \setminus N_o$, or $g$ is an edge and $g \in E_n \setminus E_o$
    \item $\alpha(g) =$ \textit{deleted} if $g$ is a node and $g \in N_o \setminus N_n$, or $g$ is an edge and $g \in E_o \setminus E_n$
    \item Otherwise, $\alpha(g) =$ \textit{remained} 
\end{itemize}

\begin{wrapfigure}{l}{0.36\textwidth}
    \centering
    \lstinputlisting[language=C]{examples/example_2.c}
    \caption{A change causing a Buffer Overflow vulnerability}
    \label{fig:example_change}
\end{wrapfigure}

To eliminate the parts irrelevant to the change, the nodes that have no path through the changed statements and their incoming and outgoing edges are removed in $G$.
%
%
%
Figure~\ref{fig:example_change} shows a commit causing a \textit{Buffer Overflow}. The CTG of the change in Figure~\ref{fig:example_change} is shown in Figure~\ref{fig:example_ctg}. As we could see from the structural change in the CTG's AST part, the condition of the \texttt{if} structure is ``relaxed" by doubling the right-hand side of the \texttt{less-than} comparison. This allows the statement at line 6 to be executed even when \texttt{len > BUF\_SIZE} (from the control flow graph). From the PDG part, the statement copies \texttt{len} (at line 3) bytes from \texttt{str} (at line 1) to \texttt{buf} (at line 2) which can have maximum \texttt{BUF\_SIZE} bytes. This will cause a overflow error when \texttt{len > BUF\_SIZE}.

After investigating more to make the set of those concepts and representations complete and accurate, we plan to develop the techniques to productively and accurately extract the representations of changes. 
The remaining research questions for this sub-tasks are:

- R5: What other kinds of information are required to understand the nature of dangerous/safe commits?

- R6: How to accurately and efficiently extract the representations of changes?

% - R7: Whether our code transformation graph effective in capture the code change features which are useful for other SE tasks other than just-in-time vulnerability detection (e.g., commit message generation or change quality estimation)

\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{imgs/ctg.png}
    \caption{The CTG corresponding to the change in Figure~\ref{fig:example_change}}
    \label{fig:example_ctg}
\end{figure}





\subsubsection{Just-In-Time Vulnerability Detection and Interpretation Framework}

This task aims to develop automated methods to identify and provide suggestions for potentially dangerous commits in different software systems based on prior knowledge of reported vulnerable commits. Then, an explanation for the suggestions will be provided for security analysis.

We plan to develop a framework for just-in-time vulnerability detection and interpretation. Figure~\ref{fig:framework} shows the overview of our idea. We plan to have three phases in our framework: \textit{training}, \textit{inferring}, and \textit{interpreting}. Each commit and the containing repository in this framework will be used to construct its CTG (described in Section~\ref{sec:ctg}). 
%
In the \textit{training} phase, the constructed CTGs are employed to learn embedding the graphs. Then, the resulting embedded vectors are fed to a classification model and learn how to discriminate between dangerous and safe commits. 
%
In the \textit{inferring} phase, the trained model classifies a commit using its embedded vector. 
%
In the \textit{interpreting} phase, the predictions and the model are interpreted to produce the code elements important for the models' decisions. These elements are refined and analyzed to identify suspicious statements using program analysis heuristics for security investigation. This leads us to the following questions, 
%
R7: What kinds of information in localizing and fixing vulnerability guideline recommendations are helpful for the developers? and
%
R8: How are the relations between the dangerous commits and the corresponding fixing commits utilized for recommending localizing/fixing guidance?
%
% This provides developers the hints for security investigation.
%
If the model determines the commit as safe, then this phase can also point out the key elements that are deemed to be safe.




\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{imgs/framework.png}
    \caption{Just-In-Time Vulnerability Detection and Interpretation Framework}
    \label{fig:framework}
\end{figure}



The remaining key research questions for in this framework are: 

R9: How to transform the nodes and edges in CTGs into vector space (graph embedding)? Whether a stand-alone graph-based pre-trained model using CTGs is suitable for just-in-time vulnerability detection and other SE tasks such as commit message generation or change quality estimation?

R10: What does the learning architecture fit the just-in-time vulnerability detection task well?

R11: Which is the most appropriate automated model interpretation strategy (e.g., black box, white box for our interpreting phase? 

% R10: What kinds of information in localizing and fixing vulnerability guideline recommendation is helpful for the developers?

% \subsubsection{Graph-based Interpretation Model}


==> problem.tex <==
Software is an important element of the infrastructure of the modern economy and society. Software vulnerability attacks target computer software systems, especially important systems such as national citizen data management, traffic, aviation coordination, and transportation. chemical/nuclear industrial operations, and national security systems, can cause significant damage. According to Veracode's survey of more than 130,000 software in 2020, more than 75\% of which contain at least one software vulnerability. Common vulnerabilities include: broken access control, cryptographic failures, SQL injections, insecure design, and wrong security configuration. According to a survey by Synopsys in 2021 with a total of 2,409 software, 97\% of the software in those software contains open source. 80\% of them contain at least one open source vulnerability. Notably, at the end of 2021, a new (zero-day) vulnerability in the popular Apache engine, Log4j was discovered. The vulnerability, known as Log4Shell (CVE-2021-44228), allows hackers to arbitrarily execute code on vulnerable servers. Many commercial cloud services are affected by this vulnerability including Amazon Web Services, Cloudflare, iCloud, Minecraft: Java version, Steam, Tencent QQ and many more. According to estimates [4], Log4Shell impacted 93\% of enterprise cloud environments. In fact, according to the latest survey of the Society for Software & Information Quality (CISQ) released in 2021, the total cost of bugs related to software vulnerabilities in the US (accounting for 33\% of the market share in the US). world technology market) by 2020 to 1.56 trillion USD. This cost accounts for 75\% of the cost caused by poor quality software.
In Vietnam, in 2021, the Ministry of Public Security recorded 8 million attack warnings with 2,763 attacks targeting the domestic electronic information system (up 26\% compared to 2020), many of which were software systems of state agencies [25]. According to statistics, more than 75\% of attacks on critical systems recorded in 2021 are exploiting hardware and software vulnerabilities [26]. Attacks to exploit such vulnerabilities can lead to damage in many ways to individuals, groups, and even affect national security. Therefore, as a part of network security, software security is increasingly concerned and determined by the Party and State in the country's development orientation, especially in the period when the country accelerates digital transformation.
To minimize the consequences caused by vulnerabilities in software, as recommended by CISQ, software vulnerabilities should be detected and fixed/prevented as soon as possible, because of late detection and correction. can cost 200 times more, or even cause more serious damage. To detect and prevent software vulnerabilities early, solutions being applied in the software industry include following safe design principles, manually reviewing security best practices. software (security best practices), and software testing. The most effective solution being applied in practice is to use techniques that automatically detect software vulnerabilities in the source code before deployment. Current automated software vulnerability detection techniques fall into two main categories: static code analysis techniques and data-driven techniques.
Static code analysis techniques including similarity-based and pattern-based such as Sonaque, Klocwork, Coverity, or Polyspace are widely used in industry. Similarity-based tools can identify vulnerabilities caused by code clones/reuses, but often produce a large number of warnings with a high false positive rate. positive). Methods using patterns require experts to define rules/features that represent vulnerabilities. This requirement makes sample methods prone to error and laborious. Therefore, an ideal method should be able to efficiently detect vulnerabilities caused by multiple causes while imposing as little reliance on human experts as possible.
Data-driven vulnerability detection using pattern regconition and machine learning provides alternative solutions for more efficient and automated vulnerability detection [15-17]. Machine learning algorithms can learn abstract patterns of potentially vulnerable source code. The researchers applied source code features such as imports, function calls, and software complexity metrics as metrics to identify likely files or pieces of code being attacked.
The emerging use of deep learning techniques provides new potential for the field of vulnerability detection using machine learning. On the one hand, the hierarchical structure of deep learning models helps to facilitate the learning of highly abstract and non-linear patterns that are capable of capturing

==> tables/tab-inspection-comparison.tex <==
\begin{table}[]
\centering
\caption{\textit{Development-process}: JIT-VL Performance Comparison}
\label{tab:vl-perf-time}
\begin{tabular}{@{}llllll@{}}
\toprule
         & top-1 & top-3 & top-5 & top-10 & MRR \\ \midrule
SN-based &       &       &       &        &     \\
JITLine &       &       &       &        &     \\
JITFine  &       &       &       &        &     \\
\tool    &       &       &       &        &     \\ \bottomrule
\end{tabular}
\end{table}

\begin{table}[]
\centering
\caption{\textit{Cross-project}: JIT-VL Comparison}
\label{tab:vl-perf-proj}
\begin{tabular}{@{}llllll@{}}
\toprule
         & top-1 & top-3 & top-5 & top-10 & MRR \\ \midrule
SN-based &       &       &       &        &     \\
JITLine &       &       &       &        &     \\
JITFine  &       &       &       &        &     \\
\tool    &       &       &       &        &     \\ \bottomrule
\end{tabular}
\end{table}

==> tasks/task1.tex <==





\subsection{Task 1: Construction of a large dataset of dangerous \& safe commits and an empirical study}
\label{sec:task_1}
This section discusses our design, preliminary results, and a plan for a user study to collect and validate a large dataset of dangerous commits of software systems' repositories.
%
To facilitate applying advanced machine learning techniques automatically and effectively learning latent and abstract dangerous commit patterns, our goal is to collect a large number of dangerous and safe commits in numerous real-world projects. Therefore, we plan to perform a semi-automated data collection process (Figure~\ref{fig:process}). 

Particularly, from various vulnerability datasets~\cite{fixing_database1,bigvul}, \textbf{(1)} we are extracting the vulnerability-fixing commits which can be considered as \textit{safe commits}~\cite{vccfinder,are_we_there,vuldigger}. 
%
To identify \textit{dangerous commits}/\textit{vulnerability contributing commits (VCCs)}, the general idea is to start from vulnerable statements and identify the commits which modify these statements. \textbf{(3)} This can be done by using \texttt{git blame}. 
%
\textbf{(2)} The vulnerable statements are identified thanks to the fixing commits based on the following heuristics. 
%
The statements which are deleted by the fixing commits could be considered to be vulnerable~\cite{vccfinder,vuldigger, vul_secret, bigvul}. 
%
For the statements added by the fixing commits, the existing studies~\cite{vccfinder,vuldigger} assume that the \textit{physically} surrounding statements are vulnerable, regardless of whether these statements semantically relate to added statements or not. This procedure could miss the actually vulnerable commits and incorrectly blame safe commits. To reduce this risk, we are starting from the statements which are \textit{semantically} related to the added statements rather than the surrounding ones.
%
Since the method of identifying vulnerable statements is based on heuristics, it could cause inaccuracy in collecting VCCs. \textbf{(4)} We plan to sample the collected commits and manually read vulnerability reports as well as source files to validate the identified VCCs, then refine our heuristics if necessary.


\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{imgs/dataset.png}
    \caption{A Semi-automated Data Collection Process}
    \label{fig:process}
\end{figure}

% \subsubsection{}
\textbf{Summarized preliminary results}. In this ongoing task, we have done Step 1 -- Step 3. In total, we have collected 14K fixing commits from the vulnerabilities reported from Jan 1990 - Aug 2022 in real-world 603 C/C++ projects such as Ffmpeg, Qemu, Linux, Chromium, and Tensorflow. There are 44K VCCs corresponding to the fixing commits. We are working on validating the heuristics used in identifying VCCs and refining our heuristics to improve the data collection procedure (Step 4). This process provides us with several observations: 


1. We found many cases violating the principle on commit matrices (e.g., developers' experience or numbers of added/deleted lines) used to detect risky commits in the existing studies~\cite{vuldigger,vccfinder}. 

2. Meanwhile, deciding if a change is dangerous/safe requires understanding certain code characteristics of not only the change but also its relevance to the unchanged parts and how the change affects code structure, execution, and dependencies. 

\textbf{Future activities}. We plan to investigate VCCs further to gain more knowledge about them. We will investigate the resolution process of VCCs by studying the corresponding fixing commits to know how they are resolved. We will examine more repositories on software vulnerabilities. Our goal is to answer the following research questions:

- R1: How complex are the vulnerabilities caused by dangerous commits (in terms of involving code statements, functions, or files)?

- R2: Which characteristics of code contribute to the riskiness/safeness of commits? 

- R3: Whether different dangerous/safe commits in different code components/projects share some similar characteristics?

==> tasks/task2.tex <==
\subsection{Task 2: Scientific Foundation for Representations, Dangerous Commit Detection, and Fine-Grained Interpretations}
\label{sec:task_1}

The goal of this task is to investigate the scientific foundation, including the concepts, representations, models, techniques, and tools to detect vulnerabilities at the commit level. Let us describe our ideas on the concepts and models to represent code changes, detect dangerous commits, and provide explanations for predictions as hints for the further interpretation of developers.

% \begin{figure}
%     \centering
%     \lstinputlisting[language=C]{examples/example.c}
%         \caption{CVE-2016-6156}
%         \label{fig:BO_vul_ex}
% \end{figure}

\subsubsection{Semantic Fine-Grained Code Transformation Representation}
\label{sec:ctg}
% In our prior work~\cite{cpathminer}, we had developed a graph-based model to represent code changes. In general, this model represents a code change by two graph method calls, variable declarations, operations, or control statements as nodes and control/data dependencies as edges. Using GROUMs, we have successfully mined object usage patterns in the programs. Usage patterns could be considered as class/method reuse and/or API reuse. Therefore, based on that model, we propose to represent vulnerability models by graphs. Each vulnerability model is a graph in which:


% 
The goal of this sub-task is to define important concepts and models to represent changes. Our key research question is R4: How to represent a code change to support understanding the change and determining its safeness/riskiness for the source code?

Based on our code-centric philosophy in just-in-time vulnerability detection and our observations from the ongoing Task 1, we plan to represent changes by the models which can capture the code semantics and the code transformation caused by the changes. The changes will be represented in the context of the unchanged parts, as well as the code transformations in the syntactic structure, execution flow, and dependencies. Once the code-centric models of the changes are built, we could employ a machine-learning model and interpreting methods to learn detecting dangerous changes and provide code-related explanations for the model's predictions.


From our point of view, a program is a set of \textit{inter-related elements} and \textit{relations} and \textit{dependencies} with other entities. The relations and dependencies of the code elements could be captured in graphs~\cite{cpathminer}. 
%
%
%
Thus, we plan to propose a graph-based representation that connects elements involved in changes when they have \textit{structural} relation, \textit{control-flowing} relation, or \textit{dependencies}. 
%
%
%
Particularly, each commit is represented as a \textit{Code Transformation Graph (CTG)} which is an annotated graph, $G = \langle N, E, \alpha \rangle$:
\begin{itemize}[noitemsep]
    \item Nodes in $N$ represent the code elements in the changed and unchanged parts.
    \item Edges in $E$ represent either the structural, control-flowing, or data/control dependency relations between nodes.
    \item Annotations for nodes and edges are either \textit{remained}, \textit{added}, or \textit{deleted} by the change. Formally, $\alpha(g) \in \{$\textit{remained}, \textit{added}, \textit{deleted}$\}$, where $g$ is a node in $N$ or an edge in $E$.
\end{itemize}
%
Our idea to construct the CTG, $G = \langle N, E, \alpha \rangle$, of a commit is combining the \textit{code property graphs (CPGs)}~\cite{cpg} of the old version ($G_o = \langle N_o, E_o \rangle$) and the new one ($G_n = \langle N_n, E_n \rangle$). By merging its \textit{abstract syntax tree (AST)}, \textit{control-flow graph (CPG)}, and \textit{program dependence graph (PDG)}, these graphs capture the syntactic structure, execution flow, and dependencies of the code \textit{version} before and the one after the commit. Specially, $G = \langle N, E, \alpha \rangle$ is constructed from $G_o = \langle N_o, E_o \rangle$ and $G_n = \langle N_n, E_n \rangle$ as follows: $N = N_o \cup N_n$, $E = E_o \cup E_n$, and for a graph element $g$ (i.e., a node or an edge of $G$):
%
\begin{itemize}[noitemsep]
    \item $\alpha(g) =$ \textit{added} if $g$ is a node and $g \in N_n \setminus N_o$, or $g$ is an edge and $g \in E_n \setminus E_o$
    \item $\alpha(g) =$ \textit{deleted} if $g$ is a node and $g \in N_o \setminus N_n$, or $g$ is an edge and $g \in E_o \setminus E_n$
    \item Otherwise, $\alpha(g) =$ \textit{remained} 
\end{itemize}

\begin{wrapfigure}{l}{0.36\textwidth}
    \centering
    \lstinputlisting[language=C]{examples/example_2.c}
    \caption{A change causing a Buffer Overflow vulnerability}
    \label{fig:example_change}
\end{wrapfigure}

To eliminate the parts irrelevant to the change, the nodes that have no path through the changed statements and their incoming and outgoing edges are removed in $G$.
%
%
%
Figure~\ref{fig:example_change} shows a commit causing a \textit{Buffer Overflow}. The CTG of the change in Figure~\ref{fig:example_change} is shown in Figure~\ref{fig:example_ctg}. As we could see from the structural change in the CTG's AST part, the condition of the \texttt{if} structure is ``relaxed" by doubling the right-hand side of the \texttt{less-than} comparison. This allows the statement at line 6 to be executed even when \texttt{len > BUF\_SIZE} (from the control flow graph). From the PDG part, the statement copies \texttt{len} (at line 3) bytes from \texttt{str} (at line 1) to \texttt{buf} (at line 2) which can have maximum \texttt{BUF\_SIZE} bytes. This will cause a overflow error when \texttt{len > BUF\_SIZE}.

After investigating more to make the set of those concepts and representations complete and accurate, we plan to develop the techniques to productively and accurately extract the representations of changes. 
The remaining research questions for this sub-tasks are:

- R5: What other kinds of information are required to understand the nature of dangerous/safe commits?

- R6: How to accurately and efficiently extract the representations of changes?

% - R7: Whether our code transformation graph effective in capture the code change features which are useful for other SE tasks other than just-in-time vulnerability detection (e.g., commit message generation or change quality estimation)

\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{imgs/ctg.png}
    \caption{The CTG corresponding to the change in Figure~\ref{fig:example_change}}
    \label{fig:example_ctg}
\end{figure}





\subsubsection{Just-In-Time Vulnerability Detection and Interpretation Framework}

This task aims to develop automated methods to identify and provide suggestions for potentially dangerous commits in different software systems based on prior knowledge of reported vulnerable commits. Then, an explanation for the suggestions will be provided for security analysis.

We plan to develop a framework for just-in-time vulnerability detection and interpretation. Figure~\ref{fig:framework} shows the overview of our idea. We plan to have three phases in our framework: \textit{training}, \textit{inferring}, and \textit{interpreting}. Each commit and the containing repository in this framework will be used to construct its CTG (described in Section~\ref{sec:ctg}). 
%
In the \textit{training} phase, the constructed CTGs are employed to learn embedding the graphs. Then, the resulting embedded vectors are fed to a classification model and learn how to discriminate between dangerous and safe commits. 
%
In the \textit{inferring} phase, the trained model classifies a commit using its embedded vector. 
%
In the \textit{interpreting} phase, the predictions and the model are interpreted to produce the code elements important for the models' decisions. These elements are refined and analyzed to identify suspicious statements using program analysis heuristics for security investigation. This leads us to the following questions, 
%
R7: What kinds of information in localizing and fixing vulnerability guideline recommendations are helpful for the developers? and
%
R8: How are the relations between the dangerous commits and the corresponding fixing commits utilized for recommending localizing/fixing guidance?
%
% This provides developers the hints for security investigation.
%
If the model determines the commit as safe, then this phase can also point out the key elements that are deemed to be safe.




\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{imgs/framework.png}
    \caption{Just-In-Time Vulnerability Detection and Interpretation Framework}
    \label{fig:framework}
\end{figure}



The remaining key research questions for in this framework are: 

R9: How to transform the nodes and edges in CTGs into vector space (graph embedding)? Whether a stand-alone graph-based pre-trained model using CTGs is suitable for just-in-time vulnerability detection and other SE tasks such as commit message generation or change quality estimation?

R10: What does the learning architecture fit the just-in-time vulnerability detection task well?

R11: Which is the most appropriate automated model interpretation strategy (e.g., black box, white box for our interpreting phase? 

% R10: What kinds of information in localizing and fixing vulnerability guideline recommendation is helpful for the developers?

% \subsubsection{Graph-based Interpretation Model}

